Denoising Implicit Feedback for Recommendation

The ubiquity of implicit feedback makes them the default choice to build online recommender systems. While the large volume of implicit feedback alleviates the data sparsity issue, the downside is that they are not as clean in reflecting the actual satisfaction of users. For example, in E-commerce, a large portion of clicks do not translate to purchases, and many purchases end up with negative reviews. As such, it is of critical importance to account for the inevitable noises in implicit feedback for recommender training. However, little work on recommendation has taken the noisy nature of implicit feedback into consideration. In this work, we explore the central theme of denoising implicit feedback for recommender training. We find serious negative impacts of noisy implicit feedback,i.e., fitting the noisy data prevents the recommender from learning the actual user preference. Our target is to identify and prune noisy interactions, so as to improve the quality of recommender training. By observing the process of normal recommender training, we find that noisy feedback typically has large loss values in the early stages. Inspired by this observation, we propose a new training strategy namedAdaptive Denoising Training(ADT), which adaptively prunes noisy interactions during training. Specifically, we devise two paradigms for adaptive loss formulation: Truncated Loss that discards the large-loss samples with a dynamic threshold in each iteration; and reweighted Loss that adaptively lowers the weight of large-loss samples. We instantiate the two paradigms on the widely used binary cross-entropy loss and test the proposed ADT strategies on three representative recommenders. Extensive experiments on three benchmarks demonstrate that ADT significantly improves the quality of recommendation over normal training.

==> NCF.tex <==
\subsection{Neural Collaborative Filtering}
Neural Collaborative Filtering (NCF) \cite{He2017Neural} is a popular CF recommendation framework, which generalizes the classic matrix factorization (MF) model by deep neural network and achieves superior performance. Different from the inner product in traditional MF methods, NCF learns an arbitrary user-item interaction function from data by non-linear neural networks. Under the NCF framework, the authors \cite{He2017Neural} proposed three neural models with different interaction functions: Generalized Matrix Factorization (GMF), Multi-Layer Perceptron (MLP), and Neural Matrix Factorization (NeuMF). 

Formally, if we use $u$ and $i$ to denote a user and an item, respectively, the interaction function of GMF can be formulated as:
%
%************************ formula 1 **************%
%
\begin{equation}
\hat{y}_{ui} = \sigma(\mathbf{h^T}(\mathbf{p_u} \odot \mathbf{p_i})),
\end{equation}
%
%************************ formula 1 **************%
%
where $\mathbf{p_u} \in \mathbb{R}^{K}$ and $\mathbf{p_u} \in \mathbb{R}^{K}$ refer to the embedding vectors of the user $u$ and the item $i$, respectively, K is the embedding size, $\mathbf{h}$ denotes the weights of the final linear layer, and $\sigma$ denotes the Sigmoid function \ie $\sigma(x) = 1/(1+e^{-x})$. Since GMF only employ one hidden layer, MLP adds more parameters to learn non-linear relationships between users and items. Its interaction function is defined as:
%
%************************ formula 2 **************%
%
\begin{equation}
\left \{
\begin{aligned}
% & \mathbf{z} = \phi_{1}(\mathbf{p_u}, \mathbf{p_i}) = [\mathbf{p_u^T}, \mathbf{p_i^T}]^T, \\
& \mathbf{z} = \phi_{1}(\mathbf{p_u}, \mathbf{p_i}) = \begin{bmatrix} \mathbf{p_u} \\   \mathbf{p_i} \end{bmatrix}, \\
& \hat{y}_{ui} = \sigma(\mathbf{h^T}\phi^{L}_{2}(\mathbf{z})),
\end{aligned}
\right .
\end{equation}
%
%************************ formula 2 **************%
%
where $\phi^{L}_{2}$ denotes a L-layer MLP model with activation functions. To model more complex user-iterm interactions well, NeuMF is proposed to fuse GMF and MLP models. The fomulation of NeuMF is obtained as follows,
%
%************************ formula 3 **************%
%
\begin{equation}
\left \{
\begin{aligned}
& \phi^{G} = \mathbf{p^{G}_u} \odot \mathbf{p^{G}_i}, \\
& \phi^{M} = \phi^{L}_{2}(\phi_{1}(\mathbf{p^{M}_u}, \mathbf{p^{M}_i})) , \\
% & \hat{y}_{ui} = \sigma(\mathbf{h^T}[\phi^{G}, \phi^{M}]^{T}),
& \hat{y}_{ui} = \sigma(\mathbf{h^T} \begin{bmatrix} \phi^{G} \\  \phi^{M} \end{bmatrix}),
\end{aligned}
\right .
\end{equation}
%
%************************ formula 3 **************%
%
where $p^{G}_u$ and $p^{G}_i$ refer to the user and item embedding of GMF, respectively; meanwhile $p^{M}_u$ and $p^{M}_i$ are similar notations for the MLP model. In this work, we choose GMF and NeuMF as the test models to justify the effectiveness of our proposed training strategy due to their superior performance.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> bu_1_intro_Jan11.tex <==
\section{Introduction}\label{sec:intro}
%%% https://www.overleaf.com/3616248989kqxfnvrdbbhf
% In the era of information explosion, recommendation systems have been widely used to discover the preferred items of users in many online services, such as E-commerce, online news and video recommendation. To train and evaluate recommendation systems, implicit interactions (\eg click) are more commonly used than explicit feedback because they are easy to acquire and partly align with the user preference. However, prior work has pointed out that there is actually a gap between the implicit interaction and the true user preference because implicit interactions (\eg click, buy and view) usually happen before the content consumption \cite{Lu2018Between, Wen2019Leveraging}. Therefore, implicit interactions are easily affected by the first impression of users and various bias, such as caption bias \cite{Lu2018Between,Lu2019effects} and position bias \cite{Jagerman2019To}. The interactions where users find they actually don't like the items are thought as negative implicit interactions. Existing studies have demonstrated the detrimental effect of negative implicit interactions on recommendation systems \cite{Lu2019effects, Wen2019Leveraging}. In this work, we prove the existence of negative effect in multiple recommendation scenarios, and then focus on the robust training of the neural recommendation models, thus reducing the influence of negative implicit interactions.
%%%%%%%%%%%%%%%%
% Jan 11 Fuli
%%%%%%%%%%%%%%%%
Neural recommenders have been the promising solution of mining user preference over items in various online services such as E-commerce~\cite{}, news portals~\cite{} and social media~\cite{}. Implicit user-item interactions (\eg click and buy) are commonly used as clues of user preference to train a neural recommender, which are easy to acquire in a large-scale. The quality of implicit interactions, \ie whether such interactions indicate true user preference, plays a crucial role in learning a reliable neural recommender. 
Unfortunately, prior work~\cite{Lu2018Between, Wen2019Leveraging} has pointed out the gap between implicit interaction and true user preference and the commonly existence of \textit{negative implicit interactions} where the user dislikes the interacted item. For instance, a large portion of buy interaction between users and items are end with negative reviews even returns. This is because implicit interactions are easily affected by users' first impression and various bias such as caption bias \cite{Lu2018Between,Lu2019effects} and position bias \cite{Jagerman2019To}. Existing studies~\cite{Lu2019effects, Wen2019Leveraging} have demonstrated the detrimental effect of such negative interactions on user experience of the online services. In this work, we investigate methods to reduce the influences of negative implicit interactions in learning a reliable neural recommender.

%******************** Figure 1 *****************%
%
\begin{figure}
\vspace{0cm}
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.4cm}
\includegraphics[scale=0.7]{images/figure1.pdf}
\caption{The comparison between the normal training of recommenders and two kinds of methods to alleviate the effect of negative interactions. One solution is to predict the user satisfaction by additional features while our method aims to prune the negative interactions during training. It's worth noting that the red lines in user-item graph denote the negative interactions.}
\label{Figure1}
\end{figure}
%
%******************* Figure 1 ***********************
%

% two ways to eliminate the effect of negative feedback
% drawbacks of the existing work
Indeed, some research efforts \cite{fox2005Evaluating, Kim2014Modeling, Yang2012Exploiting} have been dedicated to alleviating the issues of negative implicit interactions. The work falls into two categories: negative experience identification \cite{Kim2014Modeling, Lu2019effects} and the incorporation of various implicit feedback \cite{Yang2012Exploiting, Yi2014Beyond}. The former aims to predict the actual user preference by the users' behaviors (\eg dwell time and gaze pattern) and the human-designed features of recommended items (\eg the number of words and images in news). One of the problems in negative experience identification is that it has to collect various users' feedback and design different features manually to characterize the quality of items. In addition, users have to annotate if they are satisfied with the recommendation after clicks or browses. The other direction is to incorporate more implicit feedback (\eg dwell time, skip or completion) to eliminate the gap between implicit interactions and the actual user preference. For example, former studies \cite{Yi2014Beyond} find that dwell time has a strong correlation with the user satisfaction. However, various implicit feedback, especially dwell time, is not always available in general scenarios \cite{}. Even worse, most users don't give any feedback after seeing a movie or buying something \cite{}. Therefore, how to reduce the impact of negative implicit interactions on existing recommendation models without incorporating extra feedback is an untapped problem.


% challenges
% how to measure the negative effect of 

% deep learning based models black box
% how to select the clean data
% 
However, it's challenging to achieve the robust training of recommendation models without extra feedback due to the following reasons. Firstly, deep learning has revolutionized the traditional recommendation models and achieved state-of-the-art results \cite{}. While deep learning based models are able to capture more complex and valuable user-item relationships, they are hard to interpret and explain. Therefore, it's non-trivial to estimate the impact of negative implicit interactions on deep learning based recommenders. 
% It's based on the natural characteristics of  
In addition, how to identify the negative interactions and prune the user-item interactions without additional information is another tough issue. Finally, by jointly considering the superior performance of deep learning based models and the detrimental effect of negative implicit interactions, it's worth studying how to train the deep learning based recommenders well in spite of negative implicit interactions.

% Our motivation and solutions

In this paper, we find the detrimental impact of negative implicit interactions on recommendation by experiments, and then aim to alleviate the negative effect on deep learning based models. Formally, our work can be divided into three aspects: 1) exploring the effect of negative implicit interactions. Existing work has found the existence of negative implicit interactions, and summarized their detrimental impact on the user experience by some user studies. However, few work explore the effect of negative interactions on the performance of recommenders, especially the deep neural models. Since there exist negative interactions which hurt the user experience, it's unreasonable to evaluate the recommendation performance by all the interactions. Therefore, we first construct a clean test set based on some reliable feedback, such as rating scores and dwell time. For example, in the news recommendation dataset, the interactions whose dwell time is less than 10 seconds are usually treated as negative interactions \cite{}. And then we prove that the negative interactions do hurt the recommendation performance by comparing the models trained with and without negative interactions.
2) Experiments demonstrate that negative implicit interactions are ``harder'' samples for deep learning based recommenders to learn. One interesting observation for deep neural networks is the memorization effect \cite{}: deep models can learn the simple samples first, and then memorize the hard samples gradually as the training goes on. We find the same phenomenon in deep neural recommenders and the negative implicit interactions are relatively harder to learn since these items actually don't reflect the actual user preference and are usually ambiguous between interactions and skips. 3) We propose a robust training strategy for deep neural recommenders. Based on the aforementioned observations, we try to prune the user-item interactions and rank which interaction to use during training. In this work, we choose two popular collaborative filtering (CF) neural models to demonstrate the effectiveness of the proposed training strategy. And the experiments show more robust performance on three recommendation datasets.

To sum up, the contributions of our work are threefold:
\begin{itemize}[leftmargin=*]
    \item We explore the effect of negative implicit interactions on recommendation. In addition, we study the memorization effect of deep learning based recommenders and find that negative implicit interactions are harder for deep neural networks to learn.
    \item We propose a robust training strategy for deep learning based recommendation models, reducing the disturbance caused by negative implicit interactions.
    \item Experiments demonstrate that the proposed training strategy achieves effective performance improvements for two deep learning based methods on three different recommendation datasets.
\end{itemize}


% contributions
% demonstrate the negative effect in different scenarios 
% propose a robust training method to improve the existing recommendation models
% experiments demonstrated the effectiveness of the robust training method 



==> bu_1_intro_Jan12.tex <==
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%
% Jan 11 Fuli
%%%%%%%%%%%%%%%%
Neural recommenders have been the promising solution of mining user preference over items in various online services such as E-commerce~\cite{}, news portals~\cite{} and social media~\cite{}. Implicit user-item interactions (\eg click and buy) are commonly used as clues of user preference to train a neural recommender, which are easy to acquire in a large-scale. The quality of implicit interactions, \ie whether such interactions indicate actual user preference, plays a crucial role in learning a reliable neural recommender. 
Unfortunately, prior work~\cite{Lu2018Between, Wen2019Leveraging} has pointed out the gap between implicit interactions and actual user preference due to the commonly existence of \textit{negative implicit interactions} where the user dislikes the interacted item. For instance, a large portion of buy interactions between users and items are end with negative reviews even returns. This is because implicit interactions are easily affected by users' first impression and various bias such as caption bias \cite{Lu2018Between,Lu2019effects} and position bias \cite{Jagerman2019To}. Existing studies~\cite{Lu2019effects, Wen2019Leveraging} have demonstrated the detrimental effect of such negative interactions on user experience of the online services. 

In this work, we argue that the negative implicit interactions would disturb the neural recommender from learning the actual user preference, leading to biased recommendations. Table~\ref{table1} provides an empirical evidence on the detrimental effects of recommendation performance where we train NeuMF~\cite{} on two widely used recommendation datasets. In particular, we follow conventional methods~\cite{} to split each dataset into the training and testing sets, and then eliminate negative implicit interactions in testing to evaluate recommendation performance. Negative implicit interaction is identified by auxiliary information of post interaction behaviors, \eg rating score ([1, 5]) $ \le 3$, indicating that the interacted item dissatisfies the user. As can be seen, training NeuMF with noisy implicit interactions including the negative ones (\ie full training) results in an average performance drop of 23.74\% and 9.56\% \wrt Recall@20 on the two datasets as compared to the NeuMF trained without negative implicit interactions (\ie clean training). In other words, the neural recommender is biased against actual user preference by the negative implicit interactions.

%******************** Figure 1 *****************%
%
\begin{figure}
\vspace{0cm}
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.4cm}
\includegraphics[scale=0.7]{images/figure1.pdf}
\caption{The comparison between the normal training of recommenders and two kinds of methods to alleviate the effect of negative interactions. One solution is to predict the user satisfaction by additional features while our method aims to prune the negative interactions during training. It's worth noting that the red lines in user-item graph denote the negative interactions.}
\label{Figure1}
\end{figure}
%
%******************* Figure 1 ***********************
%

% two ways to eliminate the effect of negative feedback
% drawbacks of the existing work
Indeed, some research efforts \cite{fox2005Evaluating, Kim2014Modeling, Yang2012Exploiting} have been dedicated to alleviating the issues of negative implicit interactions by 1) negative experience identification~\cite{Kim2014Modeling, Lu2019effects} and 2) the incorporation of various implicit feedback \cite{Yang2012Exploiting, Yi2014Beyond} (shown in Figure~\ref{Figure1}(b)). The former could process the implicit interactions in advance by predicting the negative ones from additional user behaviors (\eg dwell time and gaze pattern) and auxiliary item features (\eg length of item description)~\cite{Lu2019effects}. % One of the problems in negative experience identification is that it has to collect various user feedback and design different features manually to characterize the quality of items. 
%In addition, users have to annotate if they are satisfied with the recommendation after clicks or browses. 
The other direction is to incorporate more types of implicit feedback (\eg dwell time and adding to the favorites) into the training of a recommender to bridge the gap between implicit interactions and actual user preference~\cite{Yi2014Beyond}. 
%For example, former studies \cite{Yi2014Beyond} find that dwell time has a strong correlation with the user satisfaction. However, various implicit feedback, especially dwell time, 
Despite the success of these methods in few specific applications~\cite{}, their usability is limited due to the unavailability of such extra users' implicit feedback in many applications such as product, food and movie recommendations. Although it might not be costly to construct mechanisms for collecting the expected feedback, these methods still face the sparse issue of such feedback. For instance, most users do not give any feedback after watching a movie or purchasing a product \cite{}. %Therefore, how to reduce the impact of negative implicit interactions on existing recommendation models without incorporating extra feedback is an untapped problem.


% challenges
% how to measure the negative effect of 

% deep learning based models black box
% how to select the clean data
% 
This work aims to learn a reliable neural recommender directly from the noisy implicit interactions, reducing the influences of negative implicit interactions without requirements of additional feedback for model training (illustrated in Figure~\ref{Figure1}).
Without extra feedback, we can only count on distilling signals of negative implicit interactions across different users and items. 
Owing to the extraordinary representativeness of deep neural networks, the neural recommender model is a concrete summary of the training data. In the training process, the model is updated at each iteration and evaluates the loss of each interaction. According to the losses, we can observe the distribution of interactions, which is a valuable signal for identifying the negative ones. According to the principal of XXX learning~\cite{}, training samples with inaccurate labels like the negative implicit interactions would be assigned outlying losses\footnote{Note that we assume the negative implicit interactions are the minority of the training interactions. Otherwise, it is unreasonable to learn a recommender from implicit feedback where most user-item interactions cannot reflect actual user preference.}. This is because, as compared to the interactions reflecting actual user preference, negative implicit interactions are more ambiguous between interactions and skips and ``harder'' to be fitted by the recommender. Nevertheless, we are still facing a tough dilemma between 1) pruning the negative implicit interactions at the beginning of training when the assigned losses could be unstable and cause misjudgement; and 2) waiting for a relatively stable loss distribution that allows the negative implicit interactions affect the early stage of training.

%Experiments demonstrate that negative implicit interactions are ``harder'' samples for deep learning based recommenders to learn. One interesting observation for deep neural networks is the memorization effect \cite{}: deep models can learn the simple samples first, and then memorize the hard samples gradually as the training goes on. We find the same phenomenon in deep neural recommenders and the negative implicit interactions are relatively harder to learn since these items actually don't reflect the actual user preference and are usually ambiguous between interactions and skips.

% Our motivation and solutions
To resolve this dilemma, we propose the robust training strategy for deep neural recommenders to learn from noisy implicit interactions. Based on the distilling signals of negative implicit interactions, we try to prune the user-item interactions and reweigh them to use during training. In this work, we design two kinds of loss functions to eliminate the effect of negative implicit interactions: Truncated Loss and Reweighted Loss. The former one adaptively truncates the contribution of large-loss instances with a dynamic threshold function in the training process. Note that the large-loss instances are more likely to be the negative implicit interactions based on the experimental findings and prior studies \cite{}. The latter loss function is to reweigh all the instance during training to avoid that the large-loss samples dominate the gradients in the process of back propagation. We have demonstrated their feasibility theoretically, and several representative neural recommenders equipped with the proposed loss functions show more robust performance on three recommendation datasets.
% In this work, we choose two popular collaborative filtering (CF) neural models to demonstrate the effectiveness of the proposed training strategy. 

Our main contributions are summarized as:
\begin{itemize}[leftmargin=*]
    \item We explore the effect of negative implicit interactions on recommendation. In addition, we study the memorization effect of deep learning based recommenders and find that negative implicit interactions are relatively harder for deep neural networks to memorize.
    \item We propose two robust loss functions for deep learning based recommendation models, reducing the disturbance caused by negative implicit interactions.
    \item Experiments demonstrate that the proposed training strategy achieves effective performance improvements for two neural recommenders on three different recommendation datasets.
\end{itemize}


% contributions
% demonstrate the negative effect in different scenarios 
% propose a robust training method to improve the existing recommendation models
% experiments demonstrated the effectiveness of the robust training method 



==> bu_1_intro_Jan16.tex <==
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%
% Jan 11 Fuli
%%%%%%%%%%%%%%%%
Neural recommenders trained with implicit feedback have been the promising solution of mining user preference over items in various online services such as E-commerce~\cite{}, news portals~\cite{} and social media~\cite{}. Implicit feedback (\eg click and purchase) is commonly used as clues of user preference to train a neural recommender because they are easy to acquire on a large-scale. Therefore, the quality of implicit feedback, \ie whether such interactions indicate the actual user preference, plays a crucial role in learning a reliable neural recommender. 
Unfortunately, prior work~\cite{Lu2018Between, Wen2019Leveraging} has pointed out the gap between implicit feedback and the actual user preference due to the common existence of \textit{noisy interactions} where the user dislikes the interacted item. For instance, a large portion of purchases end up with negative reviews even returns, and extensive clicks are followed by quits quickly. This is because implicit interactions are easily affected by users' first impressions and various biases such as caption bias \cite{Lu2018Between,Lu2019effects} and position bias \cite{Jagerman2019To}. In this work, we define these noisy interactions as \textit{false positive interactions}. Existing studies~\cite{Lu2019effects, Wen2019Leveraging} have demonstrated the detrimental effect of such false positive interactions on user experience of the online services.

In this work, we argue that such false positive interactions would disturb the neural recommender from learning the actual user preference, leading to biased recommendations. Table~\ref{table1} provides empirical evidence on the negative effects of false positive interactions where we train Neural Matrix Factorization (NeuMF)~\cite{He2017Neural} on two widely used recommendation datasets. In particular, we follow conventional methods~\cite{wang2019NGCF} to split each dataset into the training and testing sets, and then eliminate false positive interactions in the testing set to evaluate recommendation performance. Each false positive interaction is identified by auxiliary information of post-interaction behaviors, \eg rating score ([1, 5]) $ < 3$, indicating that the interacted item dissatisfies the user. As can be seen, training NeuMF with noisy implicit feedback including the false positive interactions (\ie full training) results in an average performance drop of 23.74\% and 9.56\% \wrt Recall@20 on the two datasets as compared to the NeuMF trained without false positive interactions (\ie clean training). In other words, the neural recommender is biased against the actual user preference by the false positive interactions.

%******************** Figure 1 *****************%
%
\begin{figure}
\vspace{0cm}
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{-0.4cm}
\includegraphics[scale=0.6]{images/figure1.pdf}
\caption{The comparison between the normal training of recommenders and three kinds of methods to alleviate the effect of false positive interactions. Prior solutions incorporate additional features to model the user preference while our method aims to prune the false positive interactions during training. It's worth noting that the red lines in user-item graph denote the false positive interactions.}
\label{Figure1}
\end{figure}
%
%******************* Figure 1 ***********************
%

% two ways to eliminate the effect of negative feedback
% drawbacks of the existing work
Indeed, some research efforts \cite{fox2005Evaluating, Kim2014Modeling, Yang2012Exploiting} have been dedicated to alleviating the issues of noises in implicit feedback by 1) negative experience identification~\cite{Kim2014Modeling, Lu2019effects} (illustrated in Figure~\ref{Figure1}(b)) and 2) the incorporation of various implicit feedback \cite{Yang2012Exploiting, Yi2014Beyond} (shown in Figure~\ref{Figure1}(c)). The former could process the implicit interactions in advance by predicting the false positive ones with additional user behaviors (\eg dwell time and gaze pattern) and auxiliary item features (\eg length of the item description)~\cite{Lu2019effects}. % One of the problems in negative experience identification is that it has to collect various user feedback and design different features manually to characterize the quality of items. 
%In addition, users have to annotate if they are satisfied with the recommendation after clicks or browses. 
The other direction is to incorporate more types of implicit feedback (\eg dwell time and adding to the favorites) into the training of a recommender to bridge the gap between implicit interactions and actual user preference~\cite{Yi2014Beyond}. 
%For example, former studies \cite{Yi2014Beyond} find that dwell time has a strong correlation with the user satisfaction. However, various implicit feedback, especially dwell time, 
Despite the success of these methods in some specific applications~\cite{Lu2019effects, Yang2012Exploiting, Wen2019Leveraging}, their usability is limited due to the unavailability of such extra users' implicit feedback in many applications such as product, food and movie recommendations. Although it might not be costly to construct mechanisms for collecting the expected feedback, these methods still face the sparse issue of such feedback. For instance, most users do not give any feedback after watching a movie or purchasing a product \cite{}. %Therefore, how to reduce the impact of negative implicit interactions on existing recommendation models without incorporating extra feedback is an untapped problem.


% challenges
% how to measure the negative effect of 

% deep learning based models black box
% how to select the clean data
% 
This work aims to learn a reliable neural recommender directly from the noisy implicit feedback, reducing the influences of false positive interactions without requirements of additional feedback for model training (illustrated in Figure~\ref{Figure1}(d)).
Without extra feedback, we can only count on distilling signals of false positive interactions across different users and items.
By experiments, an important observation is that the false positive interactions are ``harder'' samples for neural recommenders to memorize than true positive ones\footnote{Note that we assume the false positive interactions are the minority of the training instances. Otherwise, it is unreasonable to learn a recommender from implicit feedback where most user-item interactions cannot reflect the actual user preference.}. In particular, neural recommenders first learn the true positive user-item interactions, and ultimately overfit the false positive ones \cite{arpit2017closer, zhang2016understanding}, which is also demonstrated by the study of noisy samples in the computer vision domain \cite{lu2018MentorNet,han2018co, yu2019does}. 
Intuitively, this can be explained by that as compared to the interactions reflecting the actual user preference, false positive ones are like the noisy instances with wrong labels. Actually, they are more ambiguous between interactions and skips for users. However, although the observation provides some distilling signals for identifying false positive interactions, how to reduce their effect using these signals is still an untapped problem because the training process is dynamic and it's tough to distinguish hard samples dynamically during training.
% Owing to the extraordinary representativeness of deep neural networks, the neural recommender model is a concrete summary of the training data. In the training process, the model is updated at each iteration and evaluates the loss of each interaction. According to the losses, we can observe the distribution of interactions, which is a valuable signal for identifying the negative ones. According to the principal of XXX learning~\cite{}, training samples with inaccurate labels like the negative implicit interactions would be assigned outlying losses\footnote{Note that we assume the negative implicit interactions are the minority of the training interactions. Otherwise, it is unreasonable to learn a recommender from implicit feedback where most user-item interactions cannot reflect actual user preference.}. This is because, as compared to the interactions reflecting actual user preference, negative implicit interactions are more ambiguous between interactions and skips and ``harder'' to be fitted by the recommender. 
% Nevertheless, we are still facing a tough dilemma between 1) pruning the negative implicit interactions at the beginning of training when the assigned losses could be unstable and cause misjudgement; and 2) waiting for a relatively stable loss distribution that allows the negative implicit interactions affect the early stage of training.

%Experiments demonstrate that negative implicit interactions are ``harder'' samples for deep learning based recommenders to learn. One interesting observation for deep neural networks is the memorization effect \cite{}: deep models can learn the simple samples first, and then memorize the hard samples gradually as the training goes on. We find the same phenomenon in deep neural recommenders and the negative implicit interactions are relatively harder to learn since these items actually don't reflect the actual user preference and are usually ambiguous between interactions and skips.

% Our motivation and solutions
To resolve this issue, we propose the adaptive training strategy for deep neural recommenders to learn from noisy implicit feedback. Based on the observation about false positive interactions, we try to prune the user-item interactions and reweigh them to use during training. In this work, we design two kinds of loss functions to eliminate the effect of false positive interactions: Truncated Loss and Reweighted Loss. The former one adaptively truncates the contribution of large-loss instances (\ie hard instances) with a dynamic threshold function in the training process. Note that the large-loss instances are more likely to be false positive interactions based on our experimental findings and prior studies \cite{lu2018MentorNet, han2018co, yu2019does}. The latter loss function is to reweigh all the instances during training to avoid that the large-loss samples dominate the gradients in the process of back propagation. The core idea of the reweighted loss is to ensure that hard instances always have smaller weights than the easy ones. We have demonstrated their feasibility theoretically, and several representative neural recommenders equipped with the proposed loss functions show more robust performance on three recommendation datasets.
% In this work, we choose two popular collaborative filtering (CF) neural models to demonstrate the effectiveness of the proposed training strategy. 

Our main contributions are summarized as:
\begin{itemize}[leftmargin=*]
    \item We explore the effect of negative implicit feedback on the recommendation. In addition, we study the characteristics of false positive interactions, and find they are relatively harder for neural recommenders to memorize.
    \item To our knowledge, this is the first work to denoise implicit feedback for neural recommendation without auxiliary user behaviors. We propose two adaptive loss functions for neural recommenders, reducing the disturbance caused by false positive interactions.
    \item Experiments demonstrate that the proposed training strategy achieves effective performance improvements for three neural recommenders on three different recommendation datasets.
\end{itemize}


% contributions
% demonstrate the negative effect in different scenarios 
% propose a robust training method to improve the existing recommendation models
% experiments demonstrated the effectiveness of the robust training method 



==> bu_3_method_Jan23.tex <==

\section{Method}
In this section, we detail the proposed Adaptive Denoising Training strategy for recommenders. Prior to that, task formulation and 
%two observations about normal training for recommenders are introduced. 
observations that inspire the strategy design are introduced. 

\vspace{-0.2cm}
\subsection{\textbf{Task Formulation}}

Generally, most existing recommendation models learn user preference from implicit feedback. 
% However, there exist noisy signals because implicit interactions usually happen before content consumption, which will affect the modeling of actual user preference. 
Formally, given a training dataset $\mathcal{D} = \{(u_1, i_1, \bar{y}_{11}), (u_2, i_1, \bar{y}_{21}), ..., (u_{\textit{N}}, i_{\textit{M}}, \bar{y}_{\textit{NM}})\}$ where $\bar{y}_{ui} \in \{0, 1\}$ denotes whether implicit interactions are observed for the user $u$ and item $i$, a binary Cross-Entropy (CE) loss is usually applied to optimize the recommender's trainable parameters $\Theta_{w}$: 
%
%************************ formula 4 **************%
%
\begin{equation}
\begin{aligned}
& \mathcal{L}_{CE} = - \sum_{(u, i,  \bar{y}_{ui}) \in \mathcal{D}} \bar{y}_{ui}\log(\hat{y}_{ui}) + (1-\bar{y}_{ui})\log(1-\hat{y}_{ui}),
\end{aligned}
\end{equation}
%
%************************ formula 4 **************%
%
where $\hat{y}_{ui} \in [0,1]$ refers to the predicted score of the recommender for the user $u$ and item $i$. However, there exist noisy signals in implicit feedback because implicit interactions usually happen before content consumption. In other words, $\bar{y}_{ui}$ may not represent the true preference of the user $u$ for the item $i$. In this way, if we define $y^{\ast}_{ui} \in \{0, 1\}$ to represent whether the user $u$ really prefers the item $i$, the existence of the gap between observed implicit feedback and the true user preference can be formulated as $P(y^{\ast}_{ui}=0 | \bar{y}_{ui}=1) > 0$. Due to the inconsistency between $y^{\ast}_{ui}$ and $\bar{y}_{ui}$, the optimization for $\Theta_{w}$ is misled, leading to the biased recommender's parameters $\bar{\Theta}_{w}$ and thus poor generalization performance on the clean testing set. Differently, clean training utilizes $y^{\ast}_{ui}$ to optimize the recommender's parameters so that it produces the unbiased parameters $\Theta^{\ast}_{w}$ with the high-quality recommendation. However, the true user preference $y^{\ast}$ is usually unknown because explicit feedback and various implicit feedback from users are sparse and hard to acquire in a large quantity. 
Therefore, we aim to estimate $P(y^{\ast}_{ui}=0 | \bar{y}_{ui}=1, u, i)$ for each user-item interaction without any additional data, and then prune false-positive interactions dynamically during training. In this way, it would reduce the biased optimization, and then achieve better generalization performance on the clean testing set.


Based on the definition of $y^{\ast}_{ui}$ and $\bar{y}_{ui}$, four different types of interactions can be illustrated in Figure \ref{fig:grid}.
Although negative samples may also contain the users' preferred items, in this work, we mainly focus on denoising false-positive interactions since they would induce worse influence due to the sparsity of positive interactions.
% Note that the clean testing set only contains positive user-item interactions with label $y^{\ast}_{ui} = 1$.


%
%************************ Figure 3 **************%
%
\begin{figure}[tb]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.4cm}
\vspace{-0.2cm}
\includegraphics[scale=0.4]{images/grid.pdf}
\caption{Illustration of four different types of interactions, where the false-positive and false-negative ones denote the noisy interactions in implicit feedback.}
\label{fig:grid}
\end{figure}
%
%************************ Figure 3 **************%
%

%
%************************ Figure 2 **************%
%

\begin{figure}[ht]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.45cm}
  \centering 
  \hspace{-0.2in}
  \subfigure[Whole training process]{
    % \vspace{-0.1in}
    \label{fig2:subfig:a}
    \includegraphics[width=1.7in]{images/a20.pdf}} 
%   \hspace{-0.4in}
  \subfigure[Early training stages]{ 
    % \vspace{-0.1in}
    \label{fig2:subfig:b} 
    \includegraphics[width=1.7in]{images/a2.pdf}} 
%   \hspace{-0.5in} 
%   \vspace{-0.1in}
  \caption{The trend of the loss of true- and false-positive interactions during normal training.} 
  \label{fig:observation}
\end{figure}
%
%************************ Figure 2 **************%
%

\subsection{Observations}\label{sec:observations}
% \paragraph{{Memorization Effect of Deep Neural Networks}}
% In recent years, one interesting finding about deep neural networks is the memorization effect \cite{arpit2017closer, zhang2016understanding}. It means that if deep models have substantial capacity, they can ``memorize'' all the training data, even including the noisy samples \cite{zhang2016understanding}. However, this will lead to the poor generalization performance if the training data is unclean. In addition, deep models would first learn the simple patterns, before memorizing the noisy samples (\ie hard samples). This phenomenon happens in different neural networks (\eg MLP, CNNs, and RNNs \cite{Goodfellow2016deep}) with different optimizers (\eg Adam \cite{kingma2014adam} and Adagrad \cite{duchi2011adaptive}) and hyperparameters. 

\paragraph{{False-positive Interactions are Harder to Memorize}}
% In the previous work, researchers \cite{lu2018MentorNet, han2018co, yu2019does} have found that the noisy samples always confuse deep models and are relatively hard for them to memorize in the domain of computer vision. Actually, false-positive interactions in recommendation are similar to the noisy samples with wrongly given labels. They don't represent the users' actual interests but are thought as positive samples. Therefore, in this work, it's interesting to investigate two questions: 1) will the deep neural recommenders memorize the false-positive interactions eventually as the training goes on? And 2) are false-positive interactions harder to fit for deep models than true positive ones? 
We conduct experiments by training NeuMF with all observed implicit interactions (\ie normal training) on Adressa and Amazon-book. The loss changes of true- and false-positive interactions on Adressa are visualized in Figure \ref{fig:observation}, respectively. Similar trends are also found on Amazon-book, which is shown and discussed in section \ref{sec:memorization} to save space. From Figure \ref{fig:observation}, we have the following observations:
\begin{itemize}[leftmargin=*]
    \item The loss values of true- and false-positive interactions decrease differently in the early stages of the training process. Ultimately, the loss of both of them converges to a stable state, which implies that NeuMF memorizes both of them well. This actually reflects the memorization effect of deep neural networks~\cite{arpit2017closer, zhang2016understanding}: deep models would ``memorize'' all the training data, even including the noisy samples if they have a substantial capacity. However, it will lead to poor generalization performance if the training data is unclean.
    \item In order to highlight the learning difference between two kinds of positive interactions, we visualize the fine-grained changes of the loss \wrt iterations ranging from 0 to 1,000. From Figure \ref{fig2:subfig:b}, we can find that the loss of false-positive interactions is clearly larger than that of the true-positive ones. In addition, the difference is diminishing gradually as the training continues. The smaller loss of true-positive interactions implies that they have relatively easier patterns and can be well memorized earlier. Intuitively, true-positive interactions reflect the actual user preference and users are more certain to interact with these items. On the contrary, false-positive interactions with larger loss values are harder to memorize than the true-positive ones in the early stages of training. The reason might be that false-positive ones represent the items that the user dislikes, practically. And they are probably more similar to the items that the user doesn't interact with. Therefore, deep models are usually uncertain about the prediction of false-positive user-item pairs in the early stages. Similar conclusions about noisy samples are also found in the computer vision domain~\cite{lu2018MentorNet, han2018co, yu2019does}.
\end{itemize}

% Based on the observations, we can find that memorization effect also exists in the deep neural recommenders. They will memorize the false-positive interactions eventually, which probably can explain the poor performance of normal training in Section \ref{sec:study}. Besides, false-positive interactions are harder to memorize than the true-positive ones in early stages of training. The smaller loss of true-positive user-item interactions implies that they have relatively easier patterns and can be well memorized earlier. Intuitively, true-positive interactions reflect the actual user preference and users are more certain to interact with these items. Conversely, 


\begin{algorithm}[t]
	\caption{Adaptive Denoising training with T-CE loss}  
	\begin{algorithmic}[1]
		\Require the set of all trainable parameters $\Theta_{w}$, the training set of observed user-item interactions $\mathcal{D}$, the maximum number of iterations $T_{max}$, learning rate $\eta$, $\epsilon_{max}$, $\alpha$, $\mathcal{L}_{CE}$
		\For{$T = 1 \to T_{max}$} \algorithmiccomment{shuffle samples every epoch}
		\State \textbf{Fetch} mini-batch data $\mathcal{D}_{pos}$ from $\mathcal{D}$
		\State \textbf{Sample} unobserved interactions$\mathcal{D}_{neg}$  randomly for users in $\mathcal{D}_{pos}$ with the proportion of 1:1
		\State \textbf{Define} $\mathcal{D}_{T} = \mathcal{D}_{pos} \cup \mathcal{D}_{neg}$
		\State \textbf{Obtain} $\mathcal{\bar{D}} = \mathop{\arg\max}\limits_{\mathcal{\bar{D}}\in \mathcal{D}_{pos}, |\mathcal{\bar{D}}| = \epsilon(T)|\mathcal{D}_{T}|} \sum_{(u,i) \in \mathcal{\bar{D}}} \mathcal{L}_{CE}(u, i | \Theta_{w})$
		\State \textbf{Update} $\Theta_{w} = \Theta_{w} - \eta\nabla\frac{1}{|\mathcal{\bar{D}}|}\sum_{u,i \in \mathcal{\bar{D}}} \mathcal{L}_{CE}(u, i | \Theta_{w})$
		\State \textbf{Update} $\epsilon(T) = min(\alpha T, \epsilon_{max})$
		\EndFor 
		\Ensure the optimized parameters $\Theta_{w}$ of the recommender
	\end{algorithmic}
\end{algorithm}



\subsection{Adaptive Denoising Training}
Based on the aforementioned findings, we propose general ADT strategies for recommenders to prune false-positive interactions dynamically during training.
In particular, two paradigms are devised to formulate the loss functions: Truncated Loss and Reweighted Loss. The former is to truncate the loss values of large-loss interactions to 0 with a dynamic threshold function while the latter assigns the hard samples with smaller weights adaptively during training. In this work, we instantiate two paradigms on the widely used CE loss.

%
%************************ Figure 4 **************%
%

\begin{figure}
\vspace{0cm}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.55cm}
\includegraphics[scale=0.55]{images/loss_1.pdf}
\caption{Illustration of truncated cross-entropy loss for the observed user-item interactions (\ie samples labeled with $\bar{y}_{ui} = 1$). $T_i$ denotes the iteration number and $\tau(T_i)$ refers to the threshold function. Note that the dash area indicates the effective loss and the losses larger than $\tau(T_i)$ are truncated.}
\label{fig:truncatedloss}
\end{figure}
%
%************************ Figure 4 **************%
%


\subsubsection{\textbf{Truncated Cross-Entropy Loss}}
Since neural recommenders first learn clean and easy samples, and then memorize false-positive samples gradually, it motivates us to filter out the false-positive interactions before the models fit them.
Based on the observations in section \ref{sec:observations}, large-loss interactions are more likely to be the false-positive ones. Intuitively, we can discard the large-loss interactions to improve the anti-noise capability of deep neural recommenders.
In this section, we introduce the Truncated Cross-Entropy (shorted as T-CE) loss to adaptively discard the user-item pairs with large loss values during training. 

Formally, given a user $u$ and an item $i$, the loss function is as follows,
%
%************************ formula 5 **************%
%
\begin{equation}
\mathcal{L}_{\textit{T-CE}}(u, i) = 
\begin{cases}
0, & \mathcal{L}_{CE}(u, i) > \tau(T) \land \bar{y}_{ui}=1 \\
\mathcal{L}_{CE}(u, i), & \text{otherwise,}
\end{cases}
\end{equation}
%
%************************ formula 5 **************%
%
where $\tau(T)$ denotes a dynamic threshold function \wrt the training iteration $T$. If the CE loss for the user $u$ and the item $i$ exceeds the threshold $\tau(T)$ and the user-item pair is an observed positive interaction, this positive sample will be discarded, \ie their loss is truncated as zero. Since the loss value is decreasing with the increase of training iterations, the threshold $\tau(T)$ should become smaller correspondingly. It's worth noting that the drop rate of observed interactions is supposed to have significant positive correlations with the proportion of false-positive interactions. It implies that the threshold function $\tau(T)$ can be converted into a drop rate function $\epsilon(T)$ to achieve the T-CE loss at each iteration. According to the prior observations, the drop rate function should have the following properties: 1) all the samples will be fed into the models in the beginning so that the models can learn and distinguish the true- and false-positive interactions gradually. 2) There should be an upper bound to limit the proportion of discarded samples. Therefore, we initialize the drop rate as 0 in the beginning, set a hyper-parameter $\epsilon_{max} \in [0, 1)$ to control the maximum proportion of discarded samples, and then gradually increase the drop rate to the maximum. The increase of the drop rate can be fitted by multiple functions, such as polynomial functions and the variants of logarithm functions. In this work, we increase the drop rate in a linear fashion to reduce the hyper-parameters and simplify the function $\epsilon(T)$. In this way, the drop rate function $\epsilon(T)$ can be formulated as:
%
%************************ formula 5 **************%
%
\begin{equation}
\epsilon(T) = min(\alpha T, \epsilon_{max}),
\end{equation}
%
%************************ formula 5 **************%
%
where $\alpha$ is a hyper-parameter to adjust the pace to reach the maximum drop rate.



\subsubsection{\textbf{Reweighted Cross-Entropy Loss}}
Although the Truncated Loss adaptively reduces the influence of false-positive interactions during training, it still has at least two hyper-parameters to adjust the threshold function $\epsilon(T)$.
% suffers from the following issues: 1) the threshold function $\epsilon(T)$ is a dynamic function and thus it needs to tune several hyper-parameters to adapt to different recommenders and datasets. 2) A portion of observed positive samples are totally discarded, exacerbating the sparsity issue of positive interactions. To alleviate these problems, 
Meanwhile, we devise another paradigm (\ie Reweighted Loss) to formulate the loss function with only one hyper-parameter, assigning false-positive interactions with smaller weights adaptively along the training process. 

Formally, given a user $u$ and an item $i$, the Reweighted Cross-Entropy (R-CE) loss can be formulated as
%
%************************ formula 4 **************%
%
\begin{equation}
\nonumber
\begin{aligned}
& \mathcal{L}_{\textit{R-CE}}(u, i) = - \omega(u, i) [\bar{y}_{ui}\log(\hat{y}_{ui}) + (1-\bar{y}_{ui})\log(1-\hat{y}_{ui})],
\end{aligned}
\end{equation}
%
%************************ formula 4 **************%
%
where $\omega(u, i)$ is a weight function \wrt the user and item. Motivated by the Focal Loss \cite{lin2017focal} which incorporates the prediction probability into the weights, we define the weight function $\omega(u, i)$ as
%
%************************ formula 5 **************%
%
\begin{equation}
\omega(u, i) = 
\begin{cases}
\hat{y}_{ui}^{\beta}, & \bar{y}_{ui}=1 \\
(1-\hat{y}_{ui})^{\beta}, & \text{otherwise,}
\end{cases}
\end{equation}
%
%************************ formula 5 **************%
%
where $\beta \in [0, 1]$ is a hyper-parameter to control the variation of weights. By experiments, we find larger $\beta$ will greatly slow the optimization process, and then lead to poor performance (refer to section \ref{sec:hyperparameter} for more details.).
Since the prediction of the preference score is a binary classification problem, we can only explore the properties of R-CE loss in the following parts under the case with label $\hat{y}_{ui} = 1$, and then the other side is a symmetry problem. In addition, it's worth noting that $\hat{y}_{ui}^{\beta}$ in the weight function $\omega(u, i)$ isn't involved in computing gradients directly in the parameter optimization. It's regarded as a constant at each iteration, only affecting the weights of the samples.
Otherwise, $\hat{y}_{ui}^{\beta}$ will lead to the optimization in the opposite direction for the samples with extremely large losses, which can be found in Figure \ref{fig:reweightedloss}. Intuitively, predicting $\hat{y}_{ui} = 0$ for the samples with the label $\bar{y}_{ui}=1$ also leads to a zero loss.
The computation of gradients in R-CE loss can be formally explained as follows,
%
%************************ Figure 5 **************%
%

\begin{figure}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.4cm}
\vspace{0cm}
\includegraphics[scale=0.55]{images/loss_2.pdf}
\caption{Illustration of reweighted cross-entropy loss for the observed positive interactions. Note that the contributions of large-loss samples are greatly reduced.}
\label{fig:reweightedloss}
\end{figure}
%
%************************ Figure 5 **************%
%
%
%************************ Figure 6 **************%
%

\begin{figure}
\vspace{0cm}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.4cm}
\includegraphics[scale=0.5]{images/loss_2_factor.pdf}
\caption{The weight function with different parameters $\beta$. $\hat{y}_{ui}$ changes from 0.5 to 1 gradually along training process if $\bar{y}_{ui} = 1$ and $\beta$ controls the weight difference between hard and easy samples.}
\label{fig:beta}
\vspace{0cm}
\end{figure}
%
%************************ Figure 6 **************%
%


%
%************************ formula 6 **************%
%
\begin{equation}
\nonumber
\begin{aligned}
\frac{\partial\mathcal{L}_{\textit{R-CE}}}{\partial \Theta_{w}} & = \frac{\partial\mathcal{L}_{\textit{R-CE}}}{\partial \hat{y}_{ui}} \frac{\partial \hat{y}_{ui}}{\partial \Theta_{w}} 
= - \hat{y}_{ui}^{\beta} \frac{1}{\hat{y}_{ui}}\frac{\partial \hat{y}_{ui}}{\partial \Theta_{w}} 
= \hat{y}_{ui}^{\beta} (\frac{\partial\mathcal{L}_{\textit{CE}}}{\partial \hat{y}_{ui}} \frac{\partial \hat{y}_{ui}}{\partial \Theta_{w}}),
\end{aligned}
\end{equation}
%
%************************ formula 6 **************%
%
where $\Theta_{w}$ denotes all the trainable parameters of the neural recommender.
From Figure \ref{fig:reweightedloss}, we can see that the weight function $\omega(u, i)$ decreases the relative loss of hard samples (\ie large-loss ones) as compared to the original CE loss. In particular, the R-CE loss has the following properties:
\begin{itemize}[leftmargin=*]
    \item Both hard and easy samples are down-weighted while harder samples always have smaller weights than the easy ones. This is because the function $f(\hat{y}_{ui}) = \hat{y}_{ui}^{\beta}$ monotonically increases when $\hat{y}_{ui} \in [0, 1]$ and $\beta \in [0, 1]$, and the prediction scores of harder samples are smaller than those of the easy ones when their observed label $\bar{y}_{ui}$ is 1, which is intuitively explained in Figure \ref{fig:beta}. Therefore, false-positive interactions would be assigned smaller weights adaptively during training. In this way, it can avoid that false-positive interactions with large loss values dominate the optimization \cite{Yang2018robust}.
    \item The only hyper-parameter $\beta$ indeed controls the difference between the weights of hard and easy interactions during different training phases. In particular, if we set $\beta$ as 0, the R-CE loss will recover the traditional CE loss. Figure \ref{fig:beta} plots the function $f(\hat{y}_{ui}) = \hat{y}_{ui}^{\beta}$ under various settings of $\beta$, from which we can conclude that: 1) in the initial iterations of the training, the prediction score $\hat{y}_{ui}$ fluctuates around 0.5, and then gradually moves to 1 with the increasing weights $\hat{y}_{ui}^{\beta}$ since their observed label $\bar{y}_{ui}$ is 1. 2) $\beta$ actually decides the difference between weights of hard and easy samples. As to the same prediction scores $\hat{y}_{ui}$ for hard and easy samples, the weight difference usually becomes larger if we increase $\beta$. (\eg $d_{0.4} < d_{1.0}$ in Figure 6) 3) $\beta$ adjusts when to maximize the difference, for instance, it's in the early stages of the training if $\beta < 1$. Otherwise, the maximum difference happens in the final phase. It corresponds to the change of derivative of $f(\hat{y}_{ui})$. 4) The outliers with extremely large loss values will be assigned with very small weights, effectively improving the robustness of the models.
\end{itemize}

Due to the aforementioned properties, R-CE loss can down-weight the large-loss samples and outliers, and thereafter reduce the effect of false-positive interactions based on the former observations. 
% In addition, since neural recommenders learn true-positive interactions better than false-positive ones in the early training stage, and they ultimately memorize all the samples, it's reasonable to restrict $\beta < 1$. 
It's worth noting that the negative samples are also weighted in this paradigm because we need to ensure the loss values of all samples are within the same range, so as to prevent negative samples with large loss values from dominating the optimization. Indeed, it may provide a possible solution to alleviate the impact of false-negative interactions, which we leave in the future wok to explore.




==> bu_4_intro_Dec04.tex <==
\section{Introduction}\label{sec:intro}

Recommender systems have been a promising solution for mining user preference over items in various online services such as E-commerce~\cite{Lin2019cross}, news portals~\cite{Lu2018Between} and social media~\cite{Chen2019An}. As the clue to user choices, implicit feedback (\eg click and purchase) are typically the default choice to train a recommender due to their large volume. However, prior work~\cite{Hu2008CF, Lu2018Between, Wen2019Leveraging} points out the gap between implicit feedback and the actual user satisfaction due to the prevailing presence of \textit{noisy interactions} (\aka \textit{false-positive interactions}) where the users dislike the interacted item. For instance, in E-commerce, a large portion of purchases end up with negative reviews or being returned. This is because implicit interactions are easily affected by the first impression of users and other factors such as caption bias \cite{chen2020bias, Hofmann2012on,Lu2019effects} and position bias \cite{Jagerman2019To}. Moreover, existing studies~\cite{Lu2019effects, Wen2019Leveraging} have demonstrated the detrimental effect of such false-positive interactions on user experience of online services. Nevertheless, little work on recommendation has taken the noisy nature of implicit feedback into consideration. 

In this work, we argue that such false-positive interactions would hinder a recommender from learning the actual user preference, leading to low-quality recommendations. Table~\ref{table1} provides empirical evidence on the negative effects of false-positive interactions when we train a competitive recommender, Neural Matrix Factorization (NeuMF)~\cite{He2017Neural}, on two real-world datasets. In particular, we construct a ``clean'' testing set by removing the false-positive interactions for recommender evaluation\footnote{Each false-positive interaction is identified by auxiliary information of post-interaction behaviors, \eg rating score ([1, 5]) $ < 3$, indicating that the interacted item dissatisfies the user. Refer to Section \ref{sec:study} for more details.}. As can be seen, training NeuMF with false-positive interactions (\ie \textit{normal training}) results in an average performance drop of 16.65\% and 10.29\% over the two datasets \wrt Recall@20 and NDCG@20, as compared to the NeuMF trained without false-positive interactions (\ie \textit{clean training}). As such, it is of critical importance to account for the inevitable noises in implicit feedback and eliminate the impact of false-positive interactions for recommender training.



Indeed, some efforts \cite{fox2005Evaluating, Kim2014Modeling, Yang2012Exploiting} have been dedicated to eliminating the effects of false-positive interactions by: 1) negative experience identification~\cite{Kim2014Modeling, Lu2019effects} (illustrated in Figure~\ref{Figure1}(b)); and 2) the incorporation of various feedback \cite{Yang2012Exploiting, Yi2014Beyond} (shown in Figure~\ref{Figure1}(c)). The former processes the implicit feedback in advance by predicting the false-positive ones with additional user behaviors (\eg dwell time and gaze pattern) and auxiliary item features (\eg length of the item description)~\cite{Lu2019effects}. The latter incorporates extra feedback (\eg favorite and skip) into recommender training to prune the effects of false-positive interactions~\cite{Yi2014Beyond}. A key limitation with these methods is that they require additional data to perform denoising, which may not be easy to collect.  Moreover, extra feedback (\eg rating and favorite) is often of a smaller scale, which may suffer from the sparsity issue. For instance, many users do not give any feedback after watching a movie or purchasing a product~\cite{Hu2008CF}.



%******************** Figure 1 *****************%
%
\begin{figure}[t]
\vspace{0cm}
\setlength{\abovecaptionskip}{0.05cm}
\setlength{\belowcaptionskip}{-0.2cm}
\includegraphics[scale=0.6]{images/figure1.pdf}
\caption{The comparison between normal training (a); two prior solutions to eliminate false-positive interactions through extra data (b) and (c); and denoising training without extra data (d). Note that the red lines in the user-item graph denote false-positive interactions.}
\label{Figure1}
\end{figure}
%
%******************* Figure 1 ***********************
%

This work explores denoising implicit feedback for recommender training, which automatically reduces the influence of false-positive interactions without using any additional data (Figure~\ref{Figure1}(d)). That is, we only count on the implicit interactions and distill signals of false-positive interactions across different users and items.Prior study on robust learning~\cite{lu2018MentorNet, han2018co} and curriculum learning~\cite{Bengio2009Curriculum} demonstrate that noisy samples are relatively harder to fit into models, indicating distinct patterns of noisy samples' loss values in the training procedure. Primary experiments across different recommenders and datasets (\eg Figure~\ref{fig:observation}) reveals similar phenomenon: the loss values of false-positive interactions are larger than those of the true-positive ones in the early stages of training, while their loss values decrease to the same range at the end. Consequently, due to the larger loss, false-positive interactions can largely mislead the recommender training in the early stages. Worse still, the recommender ultimately fits the false-positive interactions due to its high representation capacity, which could be overfitting and hurt the generalization. As such, a potential idea of denoising is to reduce the impact of false-positive interactions, \eg pruning the interactions with large loss values, where the key challenge is to simultaneously decrease the sacrifice of true-positive interactions.
%To reduce the impact of false-positive interactions, a potential idea of denoising is to adaptively prune the interactions with large loss values along the training process. Considering that the training process is affected by many factors, including model, dataset, and initialization, we aim to devise a general training strategy to perform the denoising (\ie pruning) appropriately. 

% Owing to the extraordinary representativeness of deep neural networks, the neural recommender model is a concrete summary of the training data. In the training process, the model is updated at each iteration and evaluates the loss of each interaction. According to the losses, we can observe the distribution of interactions, which is a valuable signal for identifying the negative ones. According to the principal of XXX learning~\cite{}, training samples with inaccurate labels like the negative implicit interactions would be assigned outlying losses\footnote{Note that we assume the negative implicit interactions are the minority of the training interactions. Otherwise, it is unreasonable to learn a recommender from implicit feedback where most user-item interactions cannot reflect actual user preference.}. This is because, as compared to the interactions reflecting actual user preference, negative implicit interactions are more ambiguous between interactions and skips and ``harder'' to be fitted by the recommender. 
% Nevertheless, we are still facing a tough dilemma between 1) pruning the negative implicit interactions at the beginning of training when the assigned losses could be unstable and cause misjudgement; and 2) waiting for a relatively stable loss distribution that allows the negative implicit interactions affect the early stage of training.

%Experiments demonstrate that negative implicit interactions are ``harder'' samples for deep learning based recommenders to learn. One interesting observation for deep neural networks is the memorization effect \cite{}: deep models can learn the simple samples first, and then memorize the hard samples gradually as the training goes on. We find the same phenomenon in deep neural recommenders and the negative implicit interactions are relatively harder to learn since these items actually don't reflect the actual user preference and are usually ambiguous between interactions and skips.

% Our motivation and solutions
To this end, we propose Adaptive Denoising Training (ADT) strategies for recommenders, which dynamically prunes the large-loss interactions along the training process. To avoid the lost of generality, we focus only on formulating the training loss, which can be applied to any differentiable models. In detail, we devise two paradigms to formulate the training loss: 1) \textit{Truncated Loss}, which discards the large-loss interactions dynamically, and 2) \textit{Reweighted Loss}, which adaptively reweighs the interactions. For each training iteration, the Truncated Loss removes the large-loss samples (\ie hard samples) with a dynamic threshold which is automatically updated during training. 
% Inevitably, the Truncated Loss would prune true-positive interactions by mistake, especially when the portion of false-positive interactions is low. 
Besides, the Reweighted Loss dynamically assigns ``harder'' interactions with smaller weights to weaken their effects on the optimization.
We instantiate the two loss functions on the basis of the widely used binary cross-entropy loss. On three benchmarks, we test ADT trained with the Truncated Loss or Reweighted Loss over three representative recommenders: Generalized Matrix Factorization (GMF)~\cite{He2017Neural}, NeuMF~\cite{He2017Neural}, and Collaborative Denoising Auto-Encoder (CDAE)~\cite{wu2016collaborative}. The results show significant performance improvements of ADT over normal training. 
Codes and data are publicly available\footnote{\url{https://github.com/WenjieWWJ/DenoisingRec.}}.


Our main contributions are summarized as:
\begin{itemize}[leftmargin=*]
    \item We formulate the task of denoising implicit feedback for recommender training. We find the negative effect of false-positive interactions and identify their characteristics (\ie hard samples) during training.
    \item We propose Adaptive Denoising Training to prune the large-loss interactions dynamically, which introduces two paradigms to formulate the training loss: Truncated Loss and Reweighted Loss.
    \item We instantiate two paradigms on the binary cross-entropy loss and apply ADT to three representative recommenders. Extensive experiments on three benchmarks validate the effectiveness of ADT in improving the recommendation quality.
\end{itemize}

%
%************************ table 1**************%
%
\begin{table}[]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0cm}
\caption{Performance comparison between the clean training and normal training of NeuMF on Adressa and Amazon-book. \#Drop denotes the relative performance drop of normal training as compared to clean training.}
% The best results are highlighted in bold.
\label{table1}
\centering
\resizebox{0.48\textwidth}{!}{
%\setlength{\tabcolsep}{0.5mm}{
\begin{tabular}{l|cc|cc}
\hline
\textbf{Dataset}     & \multicolumn{2}{c|}{\textbf{Adressa}} & \multicolumn{2}{c}{\textbf{Amazon-book}} \\ % \hline
\textbf{Metric}      & \textbf{Recall@20}    & \textbf{NDCG@20}   & \textbf{Recall@20}   & \textbf{NDCG@20}   \\ \hline \hline
\textbf{Clean training} & 0.4040                & 0.1963             & 0.0293               & 0.0159             \\ %\hline
\textbf{Normal training}  & 0.3081                & 0.1732             & 0.0265               & 0.0145             \\ \hline
\textbf{\#Drop}      & 23.74\%               & 11.77\%            & 9.56\%               & 8.81\%             \\ \hline
\end{tabular}
%}
}
\vspace{-0.5cm}
\end{table}
%
%************************ table 1 **************%
%


==> bu_5_preliminary_Dec04.tex <==
\vspace{-0.15cm}
\section{Study on False-Positive Feedback}\label{sec:study}

The effect of noisy training samples has been studied in conventional machine learning tasks such as image classification~\cite{lu2018MentorNet, han2018co}. However, little attention has been paid to such effect on recommendation, which is inherently different from conventional tasks with training samples highly related to each other, \eg interactions on the same item.
We investigate the effects of false-positive interactions on recommender training by comparing the performance of recommenders trained with and without false-positive interactions.
An interaction is identified as false-positive or true-positive one according to the explicit feedback. For instance, a purchase is false-positive if the following rating score ([1, 5]) < 3. Although the size of such explicit feedback is typically insufficient for building robust recommenders in real-world scenarios, the scale is sufficient for a pilot experiment.
In detail, we train a competitive recommender model NeuMF under two different settings: 1) ``clean training'' which trains NeuMF on the true-positive interactions only; 
and 2) ``normal training'' which trains NeuMF on all observed user-item interactions. 
%We follow the all-ranking protocol~\cite{wang2019NGCF} to evaluate the recommendation performance on the holdout clean testing set and report Recall@20 and NDCG@20 (see more details of experiments in Section~\ref{sec:protocol}).
We evaluate the recommendation performance on the holdout clean testing set with only true-positive interactions kept, \ie the evaluation focuses on recommending more satisfying items to users. More details can be seen in Section~\ref{sec:protocol}.

% Suppose that we are able to identify false-positive interactions by reliable explicit feedback from users, we will be able to construct a ``clean'' testing set where each positive sample indicates the actual user satisfaction.
% And we compare the performance of recommenders trained with and without false-positive interactions. The superior performance implies that the model recommends more satisfying items for users. Fortunately, such reliable user feedback (\eg dwell time or rating scores) are available in a few applications, providing an opportunity for us to study the influence of false-positive interactions.

% \vspace{-0.2cm}
% \paragraph{{Dataset}}
% We conduct experiments on two datasets:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Adressa}: This is a news reading dataset~\cite{Gulla2017the} that contains the dwell time of user click on news articles. Based on the experience of former researchers \cite{Yi2014Beyond, Kim2014Modeling}, we identify the clicks with dwell time shorter than 10 seconds as false-positive interactions.
%     \item \textbf{Amazon-book}: This is a product recommendation dataset~\cite{he2016ups} which contains purchase history with rating score ranges from 1 to 5 (5 indicates the best). We intuitively treat the user-item pairs with rating scores below 3 as false-positive interactions.
% \end{itemize}

% \vspace{-0.25cm}
% \paragraph{{Settings}}

% We train a competitive recommender model NeuMF under two different settings: 1) ``clean training'' which trains NeuMF on the true-positive interactions only; 
% and 2) ``normal training'' which trains NeuMF on all observed user-item interactions. 
% We follow the all-ranking protocol~\cite{wang2019NGCF} to evaluate the recommendation performance on the holdout clean testing set and report Recall@20 and NDCG@20 (see more details of experiments in Section~\ref{sec:protocol}).

\vspace{-0.15cm}
\paragraph{Results}

Table \ref{table1} summarizes the performance of NeuMF under normal training and clean training \wrt Recall@20 and NDCG@20 on the two representative datasets, Adressa and Amazon-book. 
From Table \ref{table1}, we can observe that, as compared to the ideal setting, \ie clean training, the performance of normal training drops by 11.77\% and 8.8\% \wrt NDCG@20 on Adressa and Amazon-book, respectively. This result shows the \textit{negative effects} of false-positive interactions on recommending satisfying items to users. 
%Worse still, prior work also shows that the noise interactions will reduce the user experience~\cite{Lu2019effects}.
Worse still, recommendations from normal training have higher risk on leading to further false-positive interactions, which would hurt the user experience~\cite{Lu2019effects}.
Despite the success of clean training in the pilot study, it is not a reasonable choice in practical applications because of the sparsity issues of reliable feedback such as rating scores. 
As such, it is worth exploring denoising implicit feedback such as click, view, or buy for recommender training.

==> bu_6_method_Dec04.tex <==

\section{Method}
In this section, we detail the proposed Adaptive Denoising Training strategy for recommenders. Prior to that, task formulation and observations that inspire the strategy design are introduced. 

\vspace{-0.2cm}
\subsection{\textbf{Task Formulation}}

Generally, the target of recommender training is to learn user preference from user feedback, \ie learning a scoring function $\hat{y}_{ui} = f(u, i | \Theta)$ to assess the preference of user $u$ over item $i$ with parameters $\Theta$. Ideally, the setting of recommender training is to learn $\Theta$ from a set of reliable feedback between $N$ users ($\mathcal{U}$) and $M$ items ($\mathcal{I}$). That is, given $\mathcal{D}^{\ast} = \{(u, i, y^{\ast}_{ui}) | u \in \mathcal{U}, i \in \mathcal{I}\}$, we learn the parameters $\Theta^{\ast}$ by minimizing a recommendation loss over $\mathcal{D}^{\ast}$, \eg the binary Cross-Entropy (CE) loss:
%
%************************ formula 4 **************%
%
\begin{equation}\small\notag
\begin{aligned}%\small
& \mathcal{L}_{CE}\left(\mathcal{D}^{\ast}\right) = - \sum_{(u, i,  y^{\ast}_{ui}) \in \mathcal{D}^{\ast}} y^{\ast}_{ui}\log\left(\hat{y}_{ui}\right) + \left(1 - y^{\ast}_{ui}\right)\log\left(1-\hat{y}_{ui}\right), 
\end{aligned}
\end{equation}
%
%************************ formula 4 **************%
%
where $y^{\ast}_{ui} \in \{0, 1\}$ represents whether the user $u$ really prefers the item $i$. The recommender with $\Theta^{\ast}$ would be reliable to generate high-quality recommendations. In practice, due to the lack of large-scale reliable feedback, recommender training is typically formalized as: $\bar{\Theta} = \min \mathcal{L}_{CE}(\mathcal{\bar{D}})$, where $\mathcal{\bar{D}} = \{(u, i, \bar{y}_{ui}) | u \in \mathcal{U}, i \in \mathcal{I}\}$ is a set of implicit interactions. $\bar{y}_{ui}$ denotes whether the user $u$ has interacted with the item $i$ implicitly, such as click and purchase.

However, due to the existence of noisy interactions which would mislead the learning of user preference, the typical recommender training might result in a poor model (\ie $\bar{\Theta}$) that lacks generalization ability on the clean testing set. As such, we formulate a \textit{denoising recommender training} task as:
\begin{equation}\small
\begin{aligned}
& {\Theta}^{\ast} = \min \mathcal{L}_{CE}\big(denoise(\mathcal{\bar{D}})\big),
\end{aligned}
\end{equation}
aiming to learn a reliable recommender with parameters $\Theta^{\ast}$ by denoising implicit feedback, \ie pruning the impact of noisy interactions. Formally, by assuming the existence of inconsistency between $y^{\ast}_{ui}$  and $\bar{y}_{ui}$, we define noisy interactions as $\left\{ (u, i) | y^{\ast}_{ui}=0 \land \bar{y}_{ui}=1 \right\}$. According to the value of $y^{\ast}_{ui}$ and $\bar{y}_{ui}$, we can separate implicit feedback into four categories similar to a confusion matrix as shown in Figure~\ref{fig:grid}.
%
%************************ Figure 3 **************%
%
\begin{figure}[htb]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.4cm}
\vspace{-0.2cm}
\includegraphics[scale=0.35]{images/grid.pdf}
% \caption{Illustration of four different types of implicit interactions according to the value of user satisfaction ($y^{\ast}_{ui}$) and implicit feedback ($\bar{y}_{ui}$).}
\caption{Four types of implicit interactions.}
\label{fig:grid}
\end{figure}
%
%************************ Figure 3 **************%
%

In this work, we focus on denoising false-positive interactions and omit the false-negative ones since positive interactions are much fewer in recommendation and thus false-positive interactions would induce worse effects on recommender training. Note that we do not incorporate any additional data such as explicit feedback or reliable implicit feedback into the task of denoising, despite their success in a few applications~\cite{Wen2019Leveraging, Lu2019effects}. This is because such feedback is of a smaller scale in most cases, suffering more severely from the sparsity issue.




%
%************************ Figure 2 **************%
%

\begin{figure}[h]
\vspace{-0.2cm}
\setlength{\abovecaptionskip}{-0.10cm}
\setlength{\belowcaptionskip}{-0.5cm}
  \centering 
  \hspace{-0.2in}
  \subfigure[Whole training process]{
    % \vspace{-0.1in}
    \label{fig2:subfig:a}
    \includegraphics[width=1.5in]{images/a20.pdf}} 
%   \hspace{-0.4in}
  \subfigure[Early training stages]{ 
    % \vspace{-0.1in}
    \label{fig2:subfig:b} 
    \includegraphics[width=1.5in]{images/a2.pdf}} 
%   \hspace{-0.5in} 
%   \vspace{-0.1in}
  %\caption{The trend of the loss of true- and false-positive interactions in Adressa during the normal training of NeuMF.} 
  \caption{The training loss of true- and false-positive interactions on Adressa in the normal training of NeuMF.} 
  \label{fig:observation}
\end{figure}
%
%************************ Figure 2 **************%
%

\subsection{Observations}\label{sec:observations}

\paragraph{{False-positive interactions are harder to fit in the early stages.}}
In robust learning~\cite{lu2018MentorNet, han2018co} and curriculum learning~\cite{Bengio2009Curriculum}, one theory is that easy samples are more likely to be the clean ones and fitting the hard samples may hurt the generalization. To explore whether it also exists in recommendation, we conduct experiments by training NeuMF with all observed implicit interactions (\ie normal training) on Adressa and Amazon-book. The loss of true- and false-positive interactions in Adressa is visualized in Figure \ref{fig:observation}. 
Note that similar trends are also found over other recommenders and datasets (see more details in Section \ref{sec:memorization}). 
From Figure \ref{fig:observation}, we observe that:
\begin{itemize}[leftmargin=*]
    \item Ultimately, the loss of both of true- and false-positive interactions converges to a stable state with close values, which implies that NeuMF fits both of them well. It reflects that deep models with substantial capacity would ``memorize'' all the training data, including the noisy samples.
    % the memorization effect~\cite{arpit2017closer} of the cutting-edge neural recommenders: deep models with substantial capacity would ``memorize'' all the training data, including the noisy samples~\cite{arpit2017closer, zhang2016understanding}. 
    As such, if the data is noisy, the memorization will lead to poor generalization performance. 
    \item In the early stages of training, the loss values of true- and false-positive interactions decrease differently. 
    Furthermore, we zoom in to visualize the changes of the loss \wrt iterations ranging from 0 to 1,000 in Figure \ref{fig2:subfig:b}.
    From the figure, we can see that the loss of false-positive interactions is clearly larger than that of the true-positive ones, which indicates that 
    % The smaller loss of true-positive interactions implies that they have relatively easier patterns and can be well memorized earlier. Intuitively, true-positive interactions reflect the actual user preference and users are more certain to interact with these items. On the contrary, 
    false-positive interactions are harder to memorize than the true-positive ones in the early stages. The reason might be that false-positive ones represent the items that the user dislikes, and they are more similar to the items that the user didn't interact with (\ie the negative samples). The findings also support the prior theory in robust learning and curriculum learning~\cite{han2018co, Bengio2009Curriculum}.
    % Similar conclusions about noisy samples are also found in the computer vision domain~\cite{lu2018MentorNet, han2018co, yu2019does}, further demonstrating that the phenomenon that noisy samples are harder to fit in the early training stages isn't model-specific, data-specific, or even domain-specific.
\end{itemize}
Overall, the results are consistent with the memorization effect~\cite{arpit2017closer}: deep models will first learn the easy and clean patterns in the early stage, and eventually memorize all training samples~\cite{han2018co}.

%
%************************ Figure 4 **************%
%

\begin{figure}
\vspace{0cm}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.5cm}
\includegraphics[scale=0.4]{images/loss_1.pdf}
\caption{Illustration of T-CE loss for the observed interactions (\ie $\bar{y}_{ui} = 1$). $T_i$ is the iteration number and $\tau(T_i)$ refers to the threshold. Dash area indicates the effective loss and the loss values larger than $\tau(T_i)$ are truncated.}
\label{fig:truncatedloss}
\end{figure}
%
%************************ Figure 4 **************%
%

\subsection{Adaptive Denoising Training}

Based on the observations, we propose ADT strategies for recommenders, which estimate $P(y^{\ast}_{ui}=0 | \bar{y}_{ui}=1, u, i)$ according to the training loss. To reduce the impact of false-positive interactions, ADT dynamically prunes the large-loss interactions during training. 
In particular, ADT either \textit{discards} or \textit{reweighs} the interactions with large loss values to reduce their influences on the training objective. 
Towards this end, we devise two paradigms to formulate loss functions for denoising training:
\begin{itemize}[leftmargin=*]
\item \textit{Truncated Loss.} This is to truncate the loss values of large-loss interactions to 0 with a dynamic threshold function.
\item \textit{Reweighted Loss.} It adaptively assigns hard samples (\ie the large-loss ones) with smaller weights during training.
\end{itemize}
Note that the two paradigms formulate various recommendation loss functions, \eg CE loss, square loss~\cite{Rosasco2004are}, and BPR loss~\cite{rendle2009bpr}. In the work, we take CE loss as an example to elaborate them.





\subsubsection{\textbf{Truncated Cross-Entropy Loss}}

Functionally speaking, the Truncated Cross-Entropy (shorted as T-CE) loss discards positive interactions with large values of CE loss. Formally, we can define it as:
%
%************************ formula 5 **************%
%
\begin{equation}\small
\mathcal{L}_{\textit{T-CE}}(u, i) = 
\begin{cases}
0, & \mathcal{L}_{CE}(u, i) > \tau \land \bar{y}_{ui}=1 \\
\mathcal{L}_{CE}(u, i), & \text{otherwise,}
\end{cases}
\end{equation}
%
%************************ formula 5 **************%
%
where $\tau$ is a pre-defined threshold. The T-CE loss removes any positive interactions with CE loss larger than $\tau$ from the training. While this simple T-CE loss is easy to interpret and implement, the fixed threshold may not work properly. This is because the loss value is decreasing with the increase of training iterations. Inspired by the dynamic gradient descent methods~\cite{kingma2014adam}, we replace the fixed threshold with a dynamic threshold function $\tau(T)$ \wrt the training iteration $T$, which changes the threshold value along the training process (Figure \ref{fig:truncatedloss}).
Besides, since the loss values vary across different datasets, it would be more flexible to devise $\tau(T)$ as a function of the drop rate $\epsilon(T)$. Note that there is a bijection between the drop rate and the threshold, \ie for any training iteration, if the drop rate is given, we can calculate the threshold to filter out samples. 


Based on prior observations, a proper drop rate function should have the following properties: 
1) $\epsilon(\cdot)$ should have an upper bound to limit the proportion of discarded samples so as to prevent data missing;
2) $\epsilon(0) = 0$, \ie it should allow all the samples to be fed into the models in the beginning; 
and 3) $\epsilon(\cdot)$ should increase smoothly from zero to its upper bound, so that the model can learn and distinguish the true- and false-positive interactions gradually.

% \begin{itemize}
%     \item [1)] $\epsilon(\cdot)$ should have an upper bound to limit the proportion of discarded samples so as to prevent data missing.
%     \item [2)] $\epsilon(0) = 0$, \ie it should allow all the samples to be fed into the models in the beginning. 
%     \item [3)] $\epsilon(\cdot)$ should increase smoothly from zero to its upper bound, so that the model can learn and distinguish the true- and false-positive interactions gradually.
% \end{itemize}
% \noindent- $\epsilon(\cdot)$ should have an upper bound to limit the proportion of discarded samples so as to prevent data missing. 

% \noindent- $\epsilon(0) = 0$, \ie it should allow all the samples to be fed into the models in the beginning. 

% \noindent- $\epsilon(\cdot)$ should increase smoothly from zero to its upper bound, so that the model can learn and distinguish the true- and false-positive interactions gradually.

Towards this end, we formulate the drop rate function as:
%
%************************ formula 5 **************%
%
\begin{equation}\small
\epsilon(T) = min(\alpha T, \epsilon_{max}),
\end{equation}
%
%************************ formula 5 **************%
%
where $\epsilon_{max}$ is an upper bound and $\alpha$ is a hyper-parameter to adjust the pace to reach the maximum drop rate. Note that we increase the drop rate in a linear fashion rather than a more complex function such as a polynomial function or a logarithm function. Despite the expressiveness of these functions, they will inevitably increase the number of hyper-parameters, resulting in the increasing cost of tuning a recommender. The whole algorithm is explained in Algorithm \ref{algo:T-CE}. Note that T-CE loss discards the hard samples which are more likely to be the noisy ones. It is symmetrically contrary to the Hinge loss, and T-CE loss limits the model to be overfitting.


% \setlength{\floatsep}{-0.20cm}
\begin{algorithm}[t]
	\caption{Adaptive Denoising Training with T-CE loss}  
	\label{algo:T-CE}
	\begin{algorithmic}[1]
		\Require the set of all trainable parameters $\Theta$, the training set of observed implicit interactions $\mathcal{\bar{D}}$, the maximum number of iterations $T_{max}$, learning rate $\eta$, $\epsilon_{max}$, $\alpha$, $\mathcal{L}_{CE}$
		\For{$T = 1 \to T_{max}$} \algorithmiccomment{shuffle samples every epoch}
		\State \textbf{Fetch} mini-batch data $\mathcal{\bar{D}}_{pos}$ from $\mathcal{\bar{D}}$
		\State \textbf{Sample} unobserved interactions $\mathcal{\bar{D}}_{neg}$  randomly for users in $\mathcal{\bar{D}}_{pos}$ with the proportion of 1:1
		\State \textbf{Define} $\mathcal{\bar{D}}_{T} = \mathcal{\bar{D}}_{pos} \cup \mathcal{\bar{D}}_{neg}$
		\State \textbf{Obtain} $\mathcal{\hat{D}} = \mathop{\arg\max}\limits_{\mathcal{\hat{D}}\in \mathcal{\bar{D}}_{pos}, |\mathcal{\hat{D}}| = \epsilon(T)|\mathcal{\bar{D}}_{\textit{T}}|} \sum_{(u,i) \in \mathcal{\hat{D}}} \mathcal{L}_{CE}(u, i | \Theta_{\textit{T-1}})$
		\State \textbf{Update} $\Theta_{\textit{T}} = \Theta_{\textit{T-1}} - \eta\nabla\frac{1}{|\mathcal{\hat{D}}|}\sum_{u,i \in \mathcal{\hat{D}}} \mathcal{L}_{CE}(u, i | \Theta_{\textit{T-1}})$
		\State \textbf{Update} $\epsilon(T) = min(\alpha T, \epsilon_{max})$
		\EndFor 
		\Ensure the optimized parameters $\Theta_{T_{max}}$ of the recommender
	\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{0.1cm}





% \begin{figure}
% \setlength{\abovecaptionskip}{0cm}
% \setlength{\belowcaptionskip}{-0.5cm}
% \vspace{0cm}
% \includegraphics[scale=0.4]{images/loss_2.pdf}
% \caption{Illustration of R-CE loss for the observed positive interactions. Note that the contributions of large-loss samples are greatly reduced.}
% \label{fig:reweightedloss}
% \end{figure}
%
%************************ Figure 5 **************%
%





\subsubsection{\textbf{Reweighted Cross-Entropy Loss}}
Functionally speaking, the Reweighted Cross-Entropy (shorted as R-CE) loss down-weights the positive interactions with large loss values, which is defined as:
%
%************************ formula 4 **************%
%
\begin{equation}\small
% \nonumber
\begin{aligned}
%& \mathcal{L}_{\textit{R-CE}}(u, i) = - \omega(u, i) [\bar{y}_{ui}\log(\hat{y}_{ui}) + (1-\bar{y}_{ui})\log(1-\hat{y}_{ui})],
& \mathcal{L}_{\textit{R-CE}}(u, i) =  \omega(u, i) \mathcal{L}_{\textit{CE}}(u, i), 
\end{aligned}
\end{equation}
%
%************************ formula 4 **************%
%
where $\omega(u, i)$ is a weight function that adjusts the contribution of an observed interaction to the training objective. To achieve the target of properly down-weighting the large-loss samples, the weight function $\omega(u, i)$ is expected to have the following properties:
1) it dynamically adjusts the weights of samples during training;
2) the function will reduce the influence of a hard sample to be weaker than an easy sample;
and 3) the degree of weight reduction can be easily adjusted so that it can fit different models and datasets.


% \vspace{+1pt}
% \noindent- The function should dynamically adjust weights of samples during training.

% \noindent- The function should down-weight the influences of a hard sample (\ie large-loss interactions) to be weaker than a easy sample. 

% \noindent- The degree of weight reduction can be easily adjusted so that it can fit different models and datasets.

Inspired by the success of Focal Loss~\cite{lin2017focal}, we estimate $\omega(u, i)$ with a function of $f(\hat{y}_{ui})$ that takes the prediction score as the input. Note that the prediction score and CE loss are equivalent to identify hard samples (\ie the large-loss ones). We use the prediction score as the input of the weight function since its value is within $[0, 1]$ rather than $[0, +\infty]$, which is more accountable to further computation.
Towards this end, we formulate it as:
%
%************************ formula 5 **************%
%
\begin{equation}\small
f(\hat{y}_{ui}) = \hat{y}_{ui}^{\beta},
\end{equation}
%
%************************ formula 5 **************%
%
where $\beta \in [0, +\infty]$ is a hyper-parameter to control the range of weights. 
From Figure \ref{fig5:subfig:a}, we can see that R-CE loss equipped with the proposed weight function can significantly reduce the loss of hard samples (\ie $\hat{y}_{ui} \ll 0.5$) as compared to the original CE loss. Furthermore, the proposed weight function satisfies the aforementioned requirements:

\begin{itemize}[leftmargin=*]
    \item $f(\hat{y}_{ui}) = \hat{y}_{ui}^{\beta}$ is sensitive to  $\hat{y}_{ui}$ which is closely related to the loss value. As such, it generates dynamic weights during training.
    \item The interactions with extremely large CE loss (\eg the ``outlier'' in Figure \ref{fig5:subfig:b}) will be assigned with very small weights because $\hat{y}_{ui}$ is close to 0. Therefore, the influence of such large-loss samples is largely reduced. 
    In addition, as shown in Figure \ref{fig5:subfig:b}, harder samples always have smaller weights because the function $f(\hat{y}_{ui})$ monotonically increases when $\hat{y}_{ui} \in [0, 1]$ and $\beta \in [0, +\infty]$. As such, it can avoid that false-positive interactions with large loss values dominate the optimization during training \cite{Yang2018robust}.
    \item The hyper-parameter $\beta$ dynamically controls the gap between the weights of hard and easy samples. 
    % Figure \ref{fig5:subfig:b} plots the weight function $f(\hat{y}_{ui}) = \hat{y}_{ui}^{\beta}$ under various settings of $\beta$.
    % In Figure \ref{fig5:subfig:b}, the prediction score $\hat{y}_{ui}$ would fluctuate around 0.5 in the initial iterations of training, and then gradually move to 1 because $\bar{y}_{ui}=1$. 
    % According to the value of $\hat{y}_{ui}$, we intuitively plot four cases for initial states, easier sample, harder sample, and outlier. 
    By observing the examples in Figure \ref{fig5:subfig:b}, we can find that: 1)
    % along this process, the corresponding weight increases; And 2) 
    if $\beta$ increases, for the same pair of easy and hard samples, the gap between their weights becomes larger (\eg $d_{0.4} < d_{1.0}$ in Figure \ref{fig5:subfig:b}); and 2) if we set $\beta$ as 0, the R-CE loss will degrade to the standard CE loss. 
\end{itemize}


%Since the prediction of the preference score is a binary classification problem, we can only explore the properties of R-CE loss in the following parts under the case with label $\hat{y}_{ui} = 1$, and then the other side is a symmetry problem. 





% \begin{figure}
% \vspace{0cm}
% \setlength{\abovecaptionskip}{0cm}
% \setlength{\belowcaptionskip}{-0.6cm}
% \includegraphics[scale=0.38]{images/loss_2_factor.pdf}
% \caption{The weight function with different parameters $\beta$. $\hat{y}_{ui}$ changes from 0.5 to 1 gradually along training process if $\bar{y}_{ui} = 1$ and $\beta$ controls the weight difference between hard and easy samples.}
% \label{fig:beta}
% \vspace{0cm}
% \end{figure}
%
%************************ Figure 6 **************%
%

In practice, to ensure the loss values of all samples are within the same range, preventing negative samples with large loss values from dominating the optimization, negative samples are also weighted in this paradigm. Formally, we revise the weight function as:
%
%************************ formula 5 **************%
%
\begin{equation}
\omega(u, i) = 
\begin{cases}
\hat{y}_{ui}^{\beta}, & \bar{y}_{ui}=1 \\
(1-\hat{y}_{ui})^{\beta}, & \text{otherwise,}
\end{cases}
\end{equation}
%
%************************ formula 5 **************%
%
Indeed, it may provide a possible solution to alleviate the impact of false-negative interactions, which is left for future exploration.



% Moreover, it is worth noting that $\hat{y}_{ui}^{\beta}$ in the weight function is regarded as a constant when computing the gradients to update model parameters ($\Theta$). 
% Otherwise, it will mislead the optimization direction.
% Formally, we compute the gradient of R-CE loss \wrt $\Theta$ as follows,
% %
% %************************ formula 6 **************%
% %
% \begin{equation}
% \nonumber
% \begin{aligned}
% \frac{\partial\mathcal{L}_{\textit{R-CE}}}{\partial \Theta} & = \frac{\partial\mathcal{L}_{\textit{R-CE}}}{\partial \hat{y}_{ui}} \frac{\partial \hat{y}_{ui}}{\partial \Theta} 
% = - \hat{y}_{ui}^{\beta} \frac{1}{\hat{y}_{ui}}\frac{\partial \hat{y}_{ui}}{\partial \Theta} 
% = \hat{y}_{ui}^{\beta} (\frac{\partial\mathcal{L}_{\textit{CE}}}{\partial \hat{y}_{ui}} \frac{\partial \hat{y}_{ui}}{\partial \Theta}).
% \end{aligned}
% \end{equation}
% Note that R-CE only introduces one extra hyper-parameters ($\beta$).
% %
% %************************ formula 6 **************%
% %


\subsubsection{\textbf{In-depth Analysis}}

Since ADT depends totally on recommenders to identify false-positive interactions, one question might be whether it is reliable. Actually, many existing work~\cite{lu2018MentorNet, han2018co} has pointed out the connection between the large loss and noisy samples, and explained the underlying causality: the ``memorization'' effect of deep models. That is, deep models will first learn easy and clean patterns in the initial training phase, and then gradually memorize all samples, including noisy ones. As such, the loss of deep models in the early stage can help to filter out noisy interactions. We discuss the memorization effect of recommenders by experiments in Section \ref{sec:observations} and \ref{sec:memorization}. And the performance of T-CE loss also shows that it can 
is explored in Section \ref{sec:studyTCE}.

Another concern is that some hard samples may be more informative than easy samples and discarding hard samples would limit the model's learning ability. Indeed, as indicated in the prior studies~\cite{Bengio2009Curriculum}, hard samples in the noisy data probably confuse the model rather than help it to establish the right decision surface. As such, they may induce poor generalization. It's actually a trade-off between denoising and learning. In ADT, the $\epsilon(\cdot)$ of T-CE loss and $\beta$ of R-CE loss are to control the balance. And the sensitivity to the hyper-parameters is studied in Section \ref{sec:hyperparameter}.

==> bu_7_relatedwork_Dec04.tex <==

\section{Related Work}
This work aims to denoise implicit feedback for recommenders, which is highly related to the negative experience identification, incorporating various feedback, and the robustness of recommenders.

% \vspace{-0.2cm}
% \paragraph{\textbf{False-positive Interaction}}
% In recent years, implicit feedback (\textit{e.g.}, click and watch) has been widely used as indications of user preference in recommendation systems \cite{He2017Neural} since the collection of explicit feedback is time-consuming and possibly expensive \cite{fox2005Evaluating, Hu2008CF, Zhao2018Explicit, Gal2019When}. Even though implicit feedback is somehow correlated with user preference, 
% there exist a large proportion of noisy interactions in the implicit signals \cite{Hu2008CF, Kim2014Modeling}. 
% Many research studies have pointed out that implicit signals, especially the clicks, are easily affected by different factors, such as the position bias \cite{Jagerman2019To} and the caption bias \cite{Lu2018Between}. 
% Therefore, there is actually a gap between the implicit interaction signals and the actual user preference in various scenarios, such as news recommendation \cite{Lu2018Between, Lu2019effects}, music recommendation \cite{Yang2012Exploiting, Wen2019Leveraging}, and micro-video recommendation \cite{Wen2019Leveraging}. For example, Lu \textit{et al.} \cite{Lu2018Between} found that more than half of the click signals don't capture the actual user preference in the news recommendation. Users might be attracted by the title of news while he doesn't like its content after the click. More importantly, negative experiences are detrimental to users' following behaviors and overall satisfaction \cite{Lu2019effects}.  

% Recently, implicit feedback (\textit{e.g.}, click and watch) has been widely used to indicate the user preference in recommendation systems \cite{He2017Neural} since the collection of explicit feedback is time-consuming and expensive \cite{fox2005Evaluating, Hu2008CF, Zhao2018Explicit, Gal2019When}. Even though implicit feedback is somehow correlated with the user preference, many studies have proven that implicit signals, especially the clicks, are easily affected by many factors, such as the position bias \cite{Jagerman2019To} and the caption bias \cite{Hofmann2012on, Lu2018Between}. 
% Therefore, there exist extensive noisy interactions in various recommendation scenarios, such as news \cite{Lu2018Between, Lu2019effects}, music \cite{Yang2012Exploiting, Wen2019Leveraging}, and micro-video \cite{Wen2019Leveraging}. 
% More importantly, negative experiences are detrimental to users' following behaviors and overall satisfaction \cite{Lu2019effects}.  


\begin{figure}[tb]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0cm}
\centering 
\hspace{-0.2in}
    \subfigure[R-CE loss for the observed positive interactions. The contributions of large-loss samples are greatly reduced.]{
    % \vspace{-0.1in}
    \label{fig5:subfig:a}
    \includegraphics[width=1.5in]{images/loss_2.pdf}} 
    \hspace{0.05in}
    \subfigure[The weight function with different parameters $\beta$, where $\beta$ controls the weight difference between hard and easy samples.]{
    % \vspace{-0.2in}
    \label{fig5:subfig:b} 
    \includegraphics[width=1.8in]{images/loss_2_factor.pdf}} 
  \caption{Illustration and analysis of R-CE loss.} 
    \label{fig:R-CE}
\end{figure}
%
%************************ Figure 6 **************%
%


\vspace{-0.2cm}
\paragraph{\textbf{Negative Experience Identification}}
To reduce the gap between implicit feedback and the actual user preference, many researchers have paid attention to identify negative experiences in implicit signals \cite{fox2005Evaluating, Kim2014Modeling}. Prior work usually collects the various users' feedback (\textit{e.g.}, dwell time \cite{Kim2014Modeling}, gaze patterns \cite{Zhao2016Gaze}, and skip \cite{fox2005Evaluating}) and the item characteristics \cite{Lu2018Between, Lu2019effects} to predict the user's satisfaction. Lu \textit{et al.} \cite{Lu2018Between} predicted users' actual preference in news recommendation based on various user behaviors, news quality, and the interaction context. 
% More studies on identifying negative experiences from implicit feedback are under the web search scenario. For instance, Fox \textit{et al.} \cite{fox2005Evaluating} utilized multiple implicit users' behaviors (\textit{e.g.}, clicks, dwell time, skip or completion) to predict user satisfaction in web search. 
% In addition to the dwell time, Kim \textit{et al.} \cite{Kim2014Modeling} incorporated the features of web pages to train a click-level satisfaction model, such as topics, readability levels, and content lengths. 
However, these methods need additional feedback and extensive manual label work, \eg users have to tell if they are satisfied for each interaction. Besides, the quantification of item quality and characteristics is non-trivial \cite{Lu2018Between}, which largely relies on the manually feature design and the labeling of domain experts \cite{Lu2018Between, Lu2019effects}. The unaffordable labor cost hinders the practical usage of these methods, especially in the scenarios with constantly changing items.





\vspace{-0.2cm}
\paragraph{\textbf{Incorporating Various Feedback}}

To alleviate the impact of false-positive interactions, previous approaches \cite{liu2010understanding, Yang2012Exploiting, Yin2013silence, Gal2019When, Frolov2016Fifty} also consider incorporating more feedback (\textit{e.g.}, dwell time~\cite{Yi2014Beyond}, skip~\cite{Zhang2015adaqac, Li2019Click}, and adding to favorites) into training directly.
% For example, Yang \textit{et al.} \cite{Yang2012Exploiting} explored various positive and negative implicit feedback, such as play completion and skip, and then incorporated a new rating function with weighted feedback into the recommendation. 
% Besides, dwell time has been considered to be well correlated with the post-click user preference \cite{Yi2014Beyond, Gal2019When}. 
% Yi \textit{et al.} \cite{Yi2014Beyond} explored how to normalize dwell time, and then used them to train collaborative filtering methods. 
% Moreover, some approaches try to learn from negative feedback \cite{Zhang2015adaqac,  Frolov2016Fifty, Li2019Click, Wen2019Leveraging}. 
% Many researchers \cite{Zhang2015adaqac, Li2019Click} utilized the non-clicked query candidates as the negative samples explicitly. 
For instance, Wen \textit{et al.} \cite{Wen2019Leveraging} proposed to train the recommender using three kinds of items: ``click-complete'', ``click-skip'', and ``non-click'' ones. The last two kinds of items are both treated as negative samples but with different weights. 
However, 
% implicit feedback is easily affected by various factors \cite{Lu2018Between, Jagerman2019To}, such as the item characteristics and the interaction context. In addition, 
additional feedback might be unavailable in complex scenarios. 
For example, we cannot acquire dwell time and skip patterns after users buy products or watch movies in a cinema. Most users even don't give any informative feedback after clicks. In an orthogonal direction, this work explores denoising implicit feedback without additional information during training.

\vspace{-0.2cm}
\paragraph{\textbf{Robustness of Recommender Systems}}

Gunawardana \textit{et al.} \cite{gunawardana2015evaluating} defined the robustness of recommender systems as ``the stability of the recommendation in the presence of fake information''. Prior work \cite{Lam2004Shilling, Shriver2019Evaluating} has tried to evaluate the robustness of recommender systems under various attack methods, such as shilling attacks \cite{Lam2004Shilling} and fuzzing attacks \cite{Shriver2019Evaluating}. To build more robust recommender systems, some auto-encoder based models \cite{Florian2015Collaborative, wu2016collaborative, Liang2018Variational} introduce the denoising techniques. These approaches (\eg CDAE~\cite{wu2016collaborative}) first corrupt the interactions of user by random noises, and then try to reconstruct the original one with auto-encoders. 
%For instance, CDAE reconstructs the user preference vector based on the corrupted input and the user embedding. 
% Besides, Liang \etal \cite{Liang2018Variational} incorporated varitional autoencoder into collaborative filtering based models, showing superior performance over CDAE. 
% However, existing work usually considers the heuristic attacks or random noises, totally ignoring the natural existence of false-positive interactions in implicit feedback. The objective of this work is to verify their negative effect, and improve the robustness of neural recommenders to noisy implicit feedback.
However, these methods focus on heuristic attacks or random noises, and ignore the natural false-positive interactions in data. This work highlights the negative impact of natural noisy interactions, and improve the robustness against them.


==> bu_8_exp_Dec12.tex <==
\section{Experiment}



\paragraph{Dataset}\label{section5-1}
To evaluate the effectiveness of the proposed ADT on recommender training, we conducted experiments on three publicly accessible datasets: Adressa, Amazon-book, and Yelp. 
\begin{itemize}[leftmargin=*]
    \item \textbf{Adressa:} This is a real-world news reading dataset from Adressavisen\footnote{\url{https://www.adressa.no/}}~\cite{Gulla2017the}. It includes user clicks over news and the dwell time for each click, where the clicks with dwell time < 10s are thought of as false-positive ones~\cite{Yi2014Beyond, Kim2014Modeling}.
    \item \textbf{Amazon-book:} It is from the Amazon-review datasets\footnote{\url{http://jmcauley.ucsd.edu/data/amazon/}}~\cite{he2016ups}. It covers users' purchases over books with rating scores. A rating score below 3 is regarded as a false-positive interaction.
    \item \textbf{Yelp:} It's an open recommendation dataset\footnote{\url{https://www.yelp.com/dataset/challenge}}, in which businesses in the catering industry (\eg restaurants and bars) are reviewed by users. Similar to Amazon-book, the rating scores below 3 are regarded as false-positive feedback.
\end{itemize}

These datasets comprise the common implicit feedback: click, purchase, and consumption, which are suitable to explore the effectiveness of denoising implicit feedback although explicit feedback also exists in each interaction.
We followed former work~\cite{Liang2018Variational, wang2019NGCF, LightGCN2020he} to remove users and items with extremely sparse interactions and split the dataset into training, validation, and testing (see Table \ref{table2} for statistics). To evaluate the effectiveness of denoising implicit feedback, we kept all interactions, including the false-positive ones, in training and validation, and tested recommenders only on true-positive interactions. That is, the models are expected to recommend more satisfying items to users.
%The users and items with extremely sparse interactions are removed to ensure the data quality based on the experience of former work~\cite{Liang2018Variational, wang2019NGCF}. In addition, we first filtered out the false-positive interactions in the testing set based on reliable users' feedback, and trained the recommenders with the noisy implicit feedback. Ultimately, we evaluated their performance on the clean testing set. Note that these three datasets comprise the common implicit feedback: click, purchase, and consumption, so that they are suitable to explore the effectiveness of denoising implicit feedback. More statistics are summarized in Table \ref{table2}.


%
%************************ table 2 **************%
%
\begin{table}[t]\small
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0cm}
\caption{Statistics of the datasets. In particular, \#FP interactions refer to the number of false-positive interactions.}
\label{table2}
\centering
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{l|l|l|l|l}
\hline
Dataset      & \#User & \#Item & \#Interaction & \#FP Interaction       \\ \hline
Adressa & 212,231  & 6,596   & 419,491        & 247,628            \\ \hline
Amazon-book  & 80,464  & 98,663  & 2,714,021      & 199,475             \\ \hline
Yelp         & 45,548  & 57,396  & 1,672,520      & 260,581             \\ \hline
\end{tabular}
}
% \vspace{-0.3cm}
\end{table}
%
%************************ table 2 **************%
%
%
%************************ table 3 **************%
%
\begin{table*}[ht]
\vspace{-0.3cm}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0cm}
\caption{Overall performance of three testing recommenders trained with ADT strategies and normal training over three datasets. Note that Recall@K and NDCG@K are shorted as R@K and N@K to save space, respectively, and ``RI'' in the last column denotes the relative improvement of ADT over normal training on average. The best results are highlighted in bold.}
\label{table3}
\centering
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{l|cccc|cccc|cccc|c}
\hline
\textbf{Dataset} & \multicolumn{4}{c|}{\textbf{Adressa}} & \multicolumn{4}{c|}{\textbf{Amazon-book}} & \multicolumn{4}{c|}{\textbf{Yelp}} &  \\ %\hline
\textbf{Metric} & \textbf{R@3} & \textbf{R@20} & \textbf{N@3} & \textbf{N@20} & \textbf{R@50} & \textbf{R@100} & \textbf{N@50} & \textbf{N@100} & \textbf{R@50} & \textbf{R@100} & \textbf{N@50} & \textbf{N@100} & \textbf{RI} \\ \hline \hline
GMF & 0.0880 & 0.2141 & 0.0780 & 0.1237 & 0.0610 & 0.0953 & 0.0252 & 0.0328 & 0.0830 & 0.1344 & 0.0348 & 0.0463 & -\\ %\hline
GMF+T-CE & \textbf{0.0904} & \textbf{0.2210} & \textbf{0.0805} & \textbf{0.1275} & \textbf{0.0707} & \textbf{0.1113} & \textbf{0.0292} & \textbf{0.0382} & \textbf{0.0871} & \textbf{0.1437} & 0.0359 & \textbf{0.0486} & 8.10\% \\ %\hline
GMF+R-CE  & 0.0890 & 0.2152 & 0.0788 & 0.1248 & 0.0682 & 0.1075 & 0.0275 & 0.0362 & 0.0860 & 0.1363 & \textbf{0.0366} & 0.0480 & 5.13\% \\ \hline
NeuMF & 0.1094 & 0.3081 & 0.0947 & 0.1732 & 0.0509 & 0.0813 & 0.0210 & 0.0279 & 0.0771 & 0.1259 & 0.0317 & 0.0427 & -\\ %\hline
NeuMF+T-CE & 0.1416 & 0.3158 & 0.1267 & 0.1885 & 0.0600 & 0.0972 & 0.0240 & 0.0323 & \textbf{0.0800} & \textbf{0.1314} & \textbf{0.0325} & \textbf{0.0440} & 12.98\% \\ %\hline
NeuMF+R-CE & \textbf{0.1416} & \textbf{0.3172} & \textbf{0.1267} & \textbf{0.1900} & \textbf{0.0628} & \textbf{0.1028} & \textbf{0.0248} & \textbf{0.0334} & 0.0788 & 0.1304 & 0.0320 & 0.0436 & 14.36\% \\ \hline
CDAE & 0.1394 & 0.3208 & 0.1168 & 0.1808 & 0.0989 & 0.1507 & 0.0414 & 0.0527 & 0.1112 & 0.1732 & 0.0471 & 0.0611 &  - \\ %\hline
CDAE+T-CE & \textbf{0.1406} & \textbf{0.3220} & 0.1176 & \textbf{0.1839} & \textbf{0.1088} & \textbf{0.1645} & \textbf{0.0454} & \textbf{0.0575} & \textbf{0.1165} & \textbf{0.1806} & \textbf{0.0504} & \textbf{0.0652} & 5.36\% \\ %\hline
CDAE+R-CE & 0.1388 & 0.3164 & \textbf{0.1200} & 0.1827 & 0.1022 & 0.1560 & 0.0424 & 0.0542 & 0.1161 & 0.1801 & 0.0488 & 0.0632 & 2.46\% \\ \hline
\end{tabular}
}
\end{table*}
%
%************************ table 3 **************%
%




%For Adressa, we split the user-item interactions into the training set, validation set, and testing set according to the ratio of 8:1:1 in chronological order due to the timeliness of news. As to the other two datasets, we randomly split the observed interactions of each user according to the same ratio. Ultimately, we removed all the false-positive interactions in the testing set to ensure the reliability of the evaluation. As we use dwell time and rating to construct the clean testing set, it's the only way to evaluate if the models really recommend more satisfying items for users.


\vspace{-0.15cm}
\paragraph{Evaluation Protocols}\label{sec:protocol}
For each user in the testing set, we predicted the preference score over all the items except the positive ones used during training. 
% All the items that the user never interacts with are regarded as negative ones. 
Following existing studies \cite{He2017Neural, wang2019NGCF}, we reported the recommendation performance \wrt two widely used metrics: Recall@K and NDCG@K, where higher scores indicate better performance.
%We reported the averaged value of all users \wrt Recall and NDCG. For both of them, higher scores indicate better performance.
For both metrics, we set K as 50 and 100 for Amazon-book and Yelp, while 3 and 20 for Adressa due to its much smaller item space.
%Considering that the item number of Adressa is much smaller, we set K as 50 and 100 by default while K is 3 or 20 to evaluate the performance on Adressa. 

\vspace{-0.15cm}
\paragraph{Testing Recommenders}
To demonstrate the effectiveness of our proposed ADT strategy on denoising implicit feedback, we compared the performance of recommenders trained with T-CE or R-CE and normal training with standard CE. We selected two representative user-based neural CF models, GMF and NeuMF~\cite{He2017Neural}, and one item-based model, CDAE~\cite{wu2016collaborative}. Note that CDAE is also a representative model of robust recommender which can defend random noises within implicit feedback.
%we equipped several neural models with two paradigms, and then explore if they achieve better generalization performance on the clean testing set. We chose GMF, NeuMF, and CDAE as our testing recommenders because GMF and NeuMF are representative collaborative filtering methods, and CDAE incorporates random noises to reduce the disturbance of noisy feedback. 

%%%%%
% Added on 24 April
%%%%%
% Need to add one sentence like "we did not compare general de-noising works such as [] which are designed for tasks with inputs totally different from recommendation such as image classification"

\begin{itemize}[leftmargin=*]
    \item \textbf{GMF \cite{He2017Neural}:} This is a generalized version of matrix factorization by replacing the inner product with the element-wise product and a linear neural layer as the interaction function.
    \item \textbf{NeuMF \cite{He2017Neural}:} NeuMF is a representative CF neural model, which models the relationship between users and items by combining GMF and a Multi-Layer Perceptron (MLP). 
    \item \textbf{CDAE \cite{wu2016collaborative}:} CDAE corrupts the interactions with random noises, and then employs a MLP model to reconstruct the original input.
    % partly increasing its anti-noise capability. 
\end{itemize}
We only tested neural recommenders and omit conventional ones such as MF~\cite{koren2009matrix} and SVD++~\cite{Koren2008Factorization} due to their inferior performance~\cite{He2017Neural, wu2016collaborative}. %over conventional ones.



\vspace{-0.2cm}
\paragraph{Parameter Settings}

For the three testing recommenders, we followed their default settings, and verified the effectiveness of our methods under the same conditions. For GMF and NeuMF, the factor numbers of users and items are both 32. As to CDAE, the hidden size of MLP is set as 200. In addition, the batch size is always 1,024 and Adam~\cite{kingma2014adam} is applied to optimize all the parameters with the learning rate initialized as 0.001. As to the ADT strategies, they have three hyper-parameters in total: $\alpha$ and $\epsilon_{max}$ in T-CE loss, and $\beta$ in R-CE loss. In detail, $\epsilon_{max}$ is searched in $\{0.05, 0.1, ..., 0.5\}$ and $\beta$ is tuned in $\{0.05, 0.1, ..., 0.25, 0.5, 1.0\}$. As for $\alpha$, we controlled its range by adjusting the iteration number $\epsilon_{N}$ to the maximum drop rate $\epsilon_{max}$, and $\epsilon_{N}$ is adjusted in $\{1k, 5k, 10k, 20k, 30k\}$.

\vspace{-0.2cm}
\subsection{Performance Comparison}
Table \ref{table3} summarizes the recommendation performance comparison of the three testing models trained with standard CE, T-CE, or R-CE over three datasets. From Table \ref{table3}, we can observe:
% Three testing recommenders are trained with our proposed two paradigms to formulate the CE loss function, respectively, and Table \ref{table3} summarizes the performance comparison over three datasets. From Table \ref{table3}, we have the following observations:
\begin{itemize}[leftmargin=*]
    %\item In all cases, both the T-CE loss and R-CE loss effectively improve the performance of three testing recommenders over three datasets. For instance, the relative improvement of T-CE loss over the vanilla NeuMF is 12.98\% on average. It indicates that discarding or down-weighting hard samples during training can significantly enhance the generalization ability of neural recommenders. 
    \item In all cases, both the T-CE loss and R-CE loss effectively improve the performance, \eg NeuMF+T-CE outperforms vanilla NeuMF by 12.98\% on average over three datasets. The significant performance gain indicates the better generalization ability of neural recommenders trained by T-CE loss and R-CE loss. It validates the effectiveness of adaptive denoising training, \ie discarding or down-weighting hard samples during training. 
    % \item By comparing the T-CE Loss and R-CE Loss, we found that the T-CE loss performs better in most cases. This is because that the Reweighted Loss is still affected by the false-positive interactions even if they have smaller weights. In addition, the dynamic threshold function in the Truncated Loss can be tuned more granularly with two hyper-parameters. 
    \item By comparing the T-CE Loss and R-CE Loss, we found that the T-CE loss performs better in most cases. We postulate that the recommender still suffers from the false-positive interactions when it is trained with the Reweighted Loss, even though they have smaller weights and contribute little to the overall training loss. In addition, we suspect that the superior performance of the Truncated Loss could be attributed to the additional hyper-parameters in the dynamic threshold function which can be tuned more granularly. Further improvement might be achieved by a finer-grained user-specific or item-specific tuning of these parameters, which can be done automatically~\cite{lambdaopt}.
    \item Across the recommenders, NeuMF performs worse than GMF and CDAE, especially on Amazon-book and Yelp, which is criticized for the vulnerability to noisy interactions. Because our testing is only on the true-positive interactions, the inferior performance of NeuMF is reasonable since NeuMF with more parameters can fit more false-positive interactions during training.
    \item Both T-CE and R-CE achieve the biggest performance increase on NeuMF, which validates the effectiveness of ADT to prevent vulnerable models from the disturbance of noisy data. On the contrary, the improvement over CDAE is relatively small, showing that the design of defending random noise can also improve the robustness against false-positive interactions to some extend. Nevertheless, applying T-CE or R-CE still leads to performance gain, which further validates the rationality of denoising implicit feedback.
    %\item ADT achieves the biggest performance increase on NeuMF, and the improvement over GMF and CDAE is relatively smaller. By comparing their performance under normal training, we can find that NeuMF performs worse than GMF and CDAE, especially on Amazon-book and Yelp, indicating that NeuMF is more vulnerable to noisy interactions. The reason might be that the MLP model in NeuMF increases its complexity and makes NeuMF fit more false-positive interactions. The bigger performance improvement of ADT over NeuMF demonstrates ADT could effectively prevent vulnerable models from the disturbance of noisy data.
    % \item As to the difference over three datasets, we can observe that the biggest performance improvement is over Amazon-book while the smallest one is on Adressa. It's probably be cause that the training samples of Adressa are less, and even worse, false-positive interactions of Adressa occupies more than 59\% in all observed positive ones, which greatly affects the denoising training of neural recommenders. It implies that a great proportion of noisy interactions in the training data partly restrict the improvements of ADT.
\end{itemize}


% \begin{figure*}
% % \setlength{\abovecaptionskip}{0.2cm}
% % \setlength{\belowcaptionskip}{-0.45cm}
%   \centering 
%   \hspace{-0.5in}
%   \subfigure{
%     % \vspace{-0.1in}
%     % \label{fig:subfig:a}
%     \includegraphics[width=2in]{images/GMF_T_a_amazon.pdf}} 
%   \hspace{-0.35in}
%   \subfigure{
%     % \vspace{-0.1in}
%     % \label{fig:subfig:b} 
%     \includegraphics[width=2in]{images/GMF_T_n_amazon.pdf}} 
%   \hspace{-0.35in}
%   \subfigure{
%     % \vspace{-0.1in}
%     % \label{fig:subfig:b} 
%     \includegraphics[width=2in]{images/GMF_T_a_yelp.pdf}} 
%   \hspace{-0.35in}
%   \subfigure{
%     % \vspace{-0.1in}
%     % \label{fig:subfig:b} 
%     \includegraphics[width=2in]{images/GMF_T_n_yelp.pdf}} 
%   \hspace{-0.5in} 
%   \vspace{-0.1in}
%   \caption{.} 
%   \label{Figure7}
% \end{figure*}




% \begin{figure}
% % \setlength{\abovecaptionskip}{0.2cm}
% % \setlength{\belowcaptionskip}{-0.45cm}
%   \centering 
%   \hspace{-0.5in}
%   \subfigure{
%     \includegraphics[width=2in]{images/GMF_R_amazon.pdf}} 
%   \hspace{-0.35in}
%   \subfigure{
%     \includegraphics[width=2in]{images/GMF_R_yelp.pdf}} 
%   \hspace{-0.5in} 
%   \vspace{-0.1in}
%   \caption{.} 
%   \label{Figure8}
% \end{figure}

\noindent In the following, GMF is taken as an example to conduct thorough investigation for the consideration of computation cost.


\paragraph{Further Comparison against Using Additional Feedback}

To avoid the detrimental effect of false-positive interactions, a popular idea is to incorporate the additional user feedback for training although they are usually sparse. Existing work either adopts the additional feedback by multi-task learning \cite{Gao2019LearningTR, gao2019neural}, or leverages it to identify the true-positive interactions \cite{Wen2019Leveraging, Lu2018Between}. In this work, we introduce two classical models for comparison: Neural Multi-Task Recommendation (NMTR)~\cite{Gao2019LearningTR} and Negative feedback Re-weighting (NR)~\cite{Wen2019Leveraging}. In particular, NMTR with multi-task learning is to capture multiple user behaviors (\ie click and satisfaction) while NR uses the addition feedback (\ie dwell time and rating) to identify true-positive interactions with user satisfaction and re-weight the false-positive and non-interacted ones as negative samples. We applied NMTR and NR on the testing recommenders and reported the results of GMF in Table \ref{table4}. The results of other recommenders with similar trends are omitted to save space. 

From Table \ref{table4}, we can find that: 1) NMTR and NR achieve better performance than GMF, which validates the effectiveness of additional feedback; and 2) the results of NMTR and NR are inferior to that of ADT, both T-CE and R-CE. This is attributed to the sparsity of additional feedback. 
Indeed, the clicks with satisfaction is much fewer than the total number of clicks, and thus NR will lose extensive positive training samples. Besides, not all clicks without labeled user satisfaction indicate users' dislikes because many users seldom give explicit feedback even if they are satisfied. Therefore, treating them as negative samples will hurt the performance, which is also found by the experiments in \cite{ding2019sampler}. 


\begin{table}[]
\vspace{-0.25cm}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{0cm}
\caption{Performance \wrt GMF on Amazon-book.}
\label{table4}
\centering
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{l|cccc}
\hline
\textbf{Metric} & \textbf{R@50} & \textbf{R@100} & \textbf{N@50} & \textbf{N@100} \\ \hline \hline
{GMF} & 0.0600 & 0.0945 & 0.0247 & 0.0324 \\ \hline
{GMF+T-CE} & \textbf{0.0707} & \textbf{0.1113} & \textbf{0.0292} & \textbf{0.0382} \\ %\hline
{GMF+R-CE} & 0.0682 & 0.1075 & 0.0275 & 0.0362 \\ \hline
{GMF+NMTR} & 0.0616 & 0.0967 & 0.0254 & 0.0332 \\ %\hline
{GMF+NR} & 0.0615 & 0.0958 & 0.0254 & 0.0331  \\ \hline
\end{tabular}
}
\vspace{-0cm}
\end{table}



% \vspace{-0.15cm}
\paragraph{Performance Comparison w.r.t. Interaction Sparsity}

% Since the sparsity issue limits the preference learning of inactive users, we explored whether our ADT strategies hurt the learning of inactive users' preference because they prune many interactions during training. 
Since ADT prunes many interactions during training, we explored whether ADT hurts the preference learning of inactive users because their interacted items are sparse. 
Following the former studies~\cite{wang2019NGCF}, we split testing users into four groups according to the interaction number of each user where each group has the same number of interactions. 
%Only the results of GMF over different groups are shown in Figure \ref{fig:usergroup}. 
Figure \ref{fig:usergroup} shows the group-wise performance comparison where we can observe that the proposed ADT strategies achieve stable performance gain over normal training in all cases. It validates that ADT is also effective for the inactive users. 

\begin{figure}
\vspace{-0.6cm}
\setlength{\abovecaptionskip}{-0.2cm}
\setlength{\belowcaptionskip}{-0.2cm}
  \centering 
  \hspace{-0.5in}
  \subfigure{
    \includegraphics[width=1.8in]{images/user_group_amazon.pdf}} 
  \hspace{-0.2in}
  \subfigure{
    \includegraphics[width=1.8in]{images/user_group_yelp.pdf}} 
  \hspace{-0.5in} 
  \vspace{-0.1in}
  \caption{Performance comparison of GMF over user groups with different sparsity levels on Amazon-book and Yelp. The histograms represent the user number in each group and the lines denote the performance \wrt NDCG@100.} 
  \label{fig:usergroup}
\end{figure}


\begin{figure}
\vspace{-0.3cm}
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.05cm}
  \centering 
  \hspace{-0.6in}
  \subfigure[Normal Training]{
    \includegraphics[width=1.42in]{images/amazon-loss-normal.pdf}} 
  \hspace{-0.28in}
  \subfigure[Truncated Loss]{
    \includegraphics[width=1.42in]{images/amazon-loss-T.pdf}} 
  \hspace{-0.28in}
  \subfigure[Reweighted Loss]{
    \includegraphics[width=1.42in]{images/amazon-loss-R.pdf}} 
  \hspace{-0.6in} 
%   \vspace{-0.1in}
  \caption{Loss of GMF (a), GMF+T-CE (b) and GMF+R-CE (c).} 
%   \caption{Loss comparison of false-positive interactions between Normal Training (a), Truncated Loss (b) and Reweighted Loss (c).} 
  \label{fig:lossTrend}
\end{figure}

\begin{figure*}[ht]
\vspace{-0.2cm}
\setlength{\abovecaptionskip}{-0.5cm}
\setlength{\belowcaptionskip}{-0.35cm}
  \centering 
  \hspace{-0.6in}
  \subfigure{
    \includegraphics[width=1.3in]{images/T-a-amazon.pdf}} 
  \hspace{-0.25in}
  \subfigure{
    \includegraphics[width=1.3in]{images/T-n-amazon.pdf}} 
  \hspace{-0.25in}
  \subfigure{
    \includegraphics[width=1.3in]{images/T-a-yelp.pdf}} 
  \hspace{-0.25in}
  \subfigure{
    \includegraphics[width=1.3in]{images/T-n-yelp.pdf}} 
  \hspace{-0.25in}
  \subfigure{
    \includegraphics[width=1.3in]{images/R-amazon.pdf}} 
  \hspace{-0.25in}
  \subfigure{
    \includegraphics[width=1.3in]{images/R-yelp.pdf}} 
  \hspace{-0.6in} 
%   \vspace{-0.1in}
  \caption{Performance comparison of GMF trained with ADT on Yelp and Amazon-book \wrt different hyper-parameters.} 
  \label{fig:parameter}
\end{figure*}


\begin{figure}[t]
\vspace{-0.2cm}
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0cm}
  \centering 
  \hspace{-0.5in}
  \subfigure{
    \includegraphics[width=1.8in]{images/amazon-recall.pdf}} 
  \hspace{-0.35in}
  \subfigure{
    \includegraphics[width=1.8in]{images/amazon-precision.pdf}}
  \hspace{-0.5in} 
  \vspace{-0.1in}
  \caption{Recall and precision of false-positive interactions over GMF trained with the Truncated Loss on Amazon-book.} 
  \label{fig:recall}
\end{figure}

\vspace{-0.15cm}
\subsection{In-depth Analysis}
\vspace{-0.05cm}
\subsubsection{Memorization of False-positive Interactions}\label{sec:memorization}
%As discussed in Section \ref{sec:observations}, false-positive interactions are memorized by recommenders eventually during normal training, which leads to poor generalization performance. 
Recall that false-positive interactions are memorized by recommenders eventually under normal training, leading to poor generalization (cf. Section \ref{sec:observations}). We then investigated whether false-positive interactions are also fitted well by the recommenders trained with ADT strategies. 
Considering that the original CE loss values indicates the model's fitting ability on the samples, we depicted the CE loss of false-positive interactions during the training procedure with the real training loss as reference.
%Figure \ref{fig:lossTrend} shows the CE loss values of false-positive interactions and all training samples along the process of training GMF on Amazon-book. 



From Figure \ref{fig:lossTrend}(a), we can find that the observations in section \ref{sec:observations} also exist in the training of GMF on Amazon-book. The loss values of false-positive interactions eventually become similar to other samples, indicating that GMF fits false-positive samples well at last. On the contrary, as shown in Figure \ref{fig:lossTrend}(b), by applying T-CE, the loss values of false-positive interactions keep increasing while the overall training loss stably decreases step by step. 
%This is because the recommender always selects the small-loss samples to optimize parameters, and more and more false-positive interactions are discarded during training. 
The increased loss indicates that the recommender parameters are not optimized over the false-positive interactions, validating the capability of T-CE to identify and discard such interactions.
%3) The loss of false-positive interactions is also decreasing along the training process when GMF is trained with R-CE loss. 
As to R-CE (Figure \ref{fig:lossTrend}(c)), the loss of false-positive interactions also shows a decreasing trend, showing that the recommender still fits such interactions.
However, their loss values are still larger than the real training loss, indicating that the false-positive interactions are assigned with smaller weights by R-CE, which prevents the model from fitting them. 
Therefore, we can conclude that both paradigms reduce the effect of false-positive interactions on recommender training, which can explain their improvement over normal training.







\vspace{-0.15cm}
\subsubsection{Study of Truncated Loss}\label{sec:studyTCE}
Since the Truncated Loss achieves promising performance in the experiments, we studied how well it performs to identify and discard false-positive interactions. We first defined Recall to represent what percentage of false-positive interactions in the training data are discarded, and precision as the ratio of discarded false-positive interactions to all discarded samples. Figure \ref{fig:recall} visualizes the changes of the recall and precision along the training process. The green line in Figure \ref{fig:recall} indicates the recall and precision under the settings of random discarding. In particular, the recall of random discarding equals the drop rate during training while its precision is the proportion of noisy interactions in all training samples at each iteration. 

From Figure \ref{fig:recall}, we observed that: 1) the Truncated Loss discards nearly half of false-positive interactions after the drop rate keeps stable, greatly reducing the impact of noisy interactions; and 2) the precision of Truncated Loss is about twice as large as that of random discarding. It demonstrates that the Truncated Loss effectively utilizes the distill signals of false-positive interactions and weakens their contributions to the model training. In spite of this, we can find that a key limitation of the Truncated Loss is the low precision, \eg only 10\% precision in Figure \ref{fig:recall}, which implies that it inevitably discards many clean interactions. This also partly proves that it's worth pruning noisy interactions at the cost of losing many clean samples. And the hyper-parameters in ADT control the trade-off between denoising and losing clean samples. Besides, how to further improve the precision so as to decrease the loss of clean samples is a promising research direction in the future. 


\vspace{-0.15cm}
\subsubsection{Hyper-parameter Sensitivity}\label{sec:hyperparameter}

Our proposed ADT strategies incorporate three hyper-parameters to adjust the dynamic threshold function and the weight function in two paradigms. In particular, $\epsilon_{max}$ and $\epsilon_{N}$ are used to control the drop rate in the Truncated Loss, and $\beta$ adjusts the weight function in the Reweighted Loss. In this section, we studied how the hyper-parameters affect the performance. Only the results of GMF trained with ADT strategies on Amazon-book and Yelp are reported in Figure \ref{fig:parameter} due to space limitation. Other methods over three datasets have similar patterns. From Figure \ref{fig:parameter}, we can find that: 1) the recommender trained with the T-CE loss performs better when $\epsilon_{max} \in [0.1, 0.3]$. If $\epsilon_{max}$ exceeds 0.4, the performance drops significantly because a large proportion of samples are discarded. Therefore, the upper bound $\epsilon_{max}$ should be restricted. 2) The recommender is relatively sensitive to $\epsilon_{N}$, especially on Amazon-book, and the performance still increases when $\epsilon_{N}$ > 30k. Nevertheless, a limitation of T-CE loss is the big search space of hyper-parameters. 3) The adjustment of $\beta$ in the Reweighted Loss is consistent over different datasets, and the best results happen when $\beta$ ranges from 0.15 to 0.3. These observations provide insights on how to tune the hyper-parameters of ADT if it's applied to other recommenders and datasets.
% The $\epsilon_{N}$ controls the iterations number to reach the maximum drop rate $\epsilon_{max}$. 




==> bu_9_bib_backup.tex <==

@article{fox2005Evaluating,
  title={Evaluating Implicit Measures to Improve Web Search},
  author={Steve Fox And Kuldeep Karnawat And Mark Mydland And Susan Dumais And Thomas White},
  journal={Transactions on Information Systems},
  volume={23},
  number={2},
  pages={147-168},
  year={2005},
  publisher={ACM}
}
@inproceedings{Yang2012Exploiting,
  title={Exploiting Various Implicit Feedback for Collaborative Filtering},
  author={Byoungju Yang and Sangkeun Lee and Sungchan Park and Sang-goo Lee},
  booktitle={Proceedings of the 21st International Conference on World Wide Web},
  pages={639–640},
  year={2012},
  publisher={IW3C2}
}
@inproceedings{Yi2014Beyond,
  title={Beyond clicks: dwell time for personalization},
  author={Xing Yi and Liangjie Hong and Erheng Zhong and Nanthan Nan Liu and Suju Rajan},
  booktitle={Proceedings of the 8th Conference on Recommender Systems},
  pages={113–120},
  year={2014},
  publisher={ACM}
}
@inproceedings{Kim2014Modeling,
  title={Modeling dwell time to predict click-level satisfaction},
  author={Youngho Kim and Ahmed Hassan and Ryen W White and Imed Zitouni},
  booktitle={Proceedings of the 7th International Conference on Web Search and Data Mining},
  pages={193-202},
  year={2014},
  publisher={ACM}
}
@inproceedings{Lalmas2015Promoting,
  title={Promoting positive post-click experience for in-stream yahoo gemini users},
  author={Mounia Lalmas and Janette Lehmann and Guy Shaked and Fabrizio Silvestri, and Gabriele Tolomei},
  booktitle={Proceedings of the 21th SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={1929–1938},
  year={2015},
  publisher={ACM}
}
@inproceedings{Zhang2015adaqac,
  title={adaqac: Adaptive query auto-completion via implicit negative feedback},
  author={Aston Zhang and Amit Goyal and Weize Kong and Hongbo Deng and Anlei Dong and Yi Chang and Carl A Gunter and Jiawei Han},
  booktitle={Proceedings of the 38th International SIGIR Conference on Research and Development in Information Retrieval},
  pages={143–152},
  year={2015},
  publisher={ACM}
}
@inproceedings{Zhao2016Gaze,
  title={Gaze Prediction for Recommender Systems},
  author={Qian Zhao and Shuo Chang and F. Maxwell Harper and Joseph A. Konstan},
  booktitle={Proceedings of the 10th Conference on Recommender Systems},
  pages={131-138},
  year={2016},
  publisher={ACM}
}
@inproceedings{Zhao2018Explicit,
  title={Explicit or Implicit Feedback? Engagement or Satisfaction?},
  author={Qian Zhao and F. Maxwell Harper and Gediminas Adomavicius and Joseph A. Konstan},
  booktitle={Proceedings of the 33rd Annual Symposium on Applied Computing},
  pages={1331-1340},
  year={2018},
  publisher={ACM}
}
@inproceedings{Lu2018Between,
  title = {Between Clicks and Satisfaction: Study on Multi-Phase User Preferences and Satisfaction for Online News Reading},
  author = {Lu, Hongyu and Zhang, Min and Ma, Shaoping},
  booktitle={Proceedings of the 41st International SIGIR Conference on Research and Development in Information Retrieval},
  pages = {435--444},
  year={2018},
  publisher={ACM}
}
@inproceedings{Frolov2016Fifty,
  title = {Fifty Shades of Ratings: How to Benefit from a Negative Feedback in Top-N Recommendations Tasks},
  author = {Evgeny Frolov and Ivan Oseledets},
  booktitle={Proceedings of the 10th Conference on Recommender Systems},
  pages = {91-98},
  year={2016},
  publisher={ACM}
}
@inproceedings{Lu2019effects,
  title = {Effects of User Negative Experience in Mobile News Streaming},
  author = {Lu, Hongyu and Zhang, Min and Ma, Weizhi and Wang, Ce and xia, Feng and Liu, Yiqun and Lin, Leyu and Ma, Shaoping},
  booktitle={Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages = {705--714},
  year={2019},
  publisher={ACM}
}
@inproceedings{Jagerman2019To,
  title = {To Model or to Intervene: A Comparison of Counterfactual and Online Learning to Rank from User Interactions},
  author = {Rolf Jagerman and Harrie Oosterhuis and Maarten de Rijke},
  booktitle={Proceedings of the 42nd International SIGIR Conference on Research and Development in Information Retrieval},
  pages = {15-24},
  year={2019},
  publisher={ACM}
}
@inproceedings{Wen2019Leveraging,
  title = {Leveraging Post-click Feedback for Content Recommendations},
  author = {Wen, Hongyi and Yang, Longqi and Estrin, Deborah},
  booktitle = {Proceedings of the 13th Conference on Recommender Systems},
  pages = {278--286},
  year={2019},
  publisher={ACM}
}
@inproceedings{Li2019Click,
  title = {Click Feedback-Aware Query Recommendation Using Adversarial Examples},
  author = {Li, Ruirui and Li, Liangda and Wu, Xian and Zhou, Yunhong and Wang, Wei},
  booktitle={Proceedings of the 28th International Conference on World Wide Web},
  pages = {2978-2984},
  year={2019},
  publisher={IW3C2}
}
@inproceedings{He2017Neural,
  title = {Neural Collaborative Filtering},
  author = {He, Xiangnan and Liao, Lizi and Zhang, Hanwang and Nie, Liqiang and Hu, Xia and Chua, Tat-Seng},
  booktitle={Proceedings of the 26th International Conference on World Wide Web},
  pages = {173--182},
  year={2017},
  publisher={IW3C2}
}
@inproceedings{Gal2019When,
  title = {When Actions Speak Louder Than Clicks: A Combined Model of Purchase Probability and Long-term Customer Satisfaction},
  author = {Lavee, Gal and Koenigstein, Noam and Barkan, Oren},
  booktitle = {Proceedings of the 13th Conference on Recommender Systems},
  pages = {287--295},
  year={2019},
  publisher={ACM}
}
@incollection{gunawardana2015evaluating,
  title={Evaluating Recommender Systems},
  author={Gunawardana, Asela and Shani, Guy},
  booktitle={Recommender Systems handbook},
  pages={265--308},
  year={2015},
  publisher={Springer}
}

@inproceedings{Lam2004Shilling,
  author = {Lam, Shyong K. and Riedl, John},
  title = {Shilling Recommender Systems for Fun and Profit},
  booktitle = {Proceedings of the 13th International Conference on World Wide Web},
  year = {2004},
  pages = {393--402},
  publisher={IW3C2}
}

@inproceedings{Shriver2019Evaluating,
  title = {Evaluating Recommender System Stability with Influence-Guided Fuzzing},
  author={David Shriver and Sebastian G. Elbaum and Matthew B. Dwyer and David S. Rosenblum},
  booktitle={Proceedings of the 33rd {AAAI} Conference on Artificial Intelligence},
  year={2019},
  pages = {4934--4942},
  publisher = {{AAAI} Press}
}

@inproceedings{Florian2015Collaborative,
  title={Collaborative Filtering with Stacked Denoising AutoEncoders and Sparse Inputs},
  author={Strub, Florian and Mary, Jeremie},
  booktitle={Workshop of Neural Information Processing Systems},
  year={2015},
  organization = {MIT Press}
}

@inproceedings{wu2016collaborative,
  title={Collaborative denoising auto-encoders for top-n Recommender Systems},
  author={Wu, Yao and DuBois, Christopher and Zheng, Alice X and Ester, Martin},
  booktitle={Proceedings of the 9th International Conference on Web Search and Data Mining},
  pages={153--162},
  year={2016},
  organization={ACM}
}
@inproceedings{Liang2018Variational,
 author = {Liang, Dawen and Krishnan, Rahul G. and Hoffman, Matthew D. and Jebara, Tony},
 title = {Variational Autoencoders for Collaborative Filtering},
 booktitle = {Proceedings of the 27th International Conference on World Wide Web},
 year = {2018},
 pages = {689--698},
 publisher = {IW3C2},
} 
@inproceedings{wang2019NGCF,
  author    = {Xiang Wang and
               Xiangnan He and
               Meng Wang and
               Fuli Feng and
               Tat{-}Seng Chua},
  title     = {Neural Graph Collaborative Filtering},
  booktitle = {Proceedings of the 42nd International SIGIR Conference on Research and Development in Information Retrieval},
  pages     = {165--174},
  year      = {2019},
  publisher={ACM}
}
@inproceedings{han2018co,
  title={Co-teaching: Robust training of deep neural networks with extremely noisy labels},
  author={Han, Bo and Yao, Quanming and Yu, Xingrui and Niu, Gang and Xu, Miao and Hu, Weihua and Tsang, Ivor and Sugiyama, Masashi},
  publisher = {Curran Associates Inc.},
  booktitle = {Proceedings of the 32nd International Conference on Neural Information Processing Systems},
  pages={8527--8537},
  year={2018},
  organization = {MIT Press}
}
@inproceedings{yu2019does,
  title={How does Disagreement Help Generalization against Label Corruption?},
  author={Yu, Xingrui and Han, Bo and Yao, Jiangchao and Niu, Gang and Tsang, Ivor and Sugiyama, Masashi},
  booktitle={Proceedings of the 36th International Conference on Machine Learning},
  pages={7164--7173},
  year={2019},
  publisher = {PMLR},
}
@inproceedings{lu2018MentorNet,
  title={MentorNet: Learning Data-Driven Curriculum for Very Deep Neural Networks on Corrupted Labels},
  author={Jiang, Lu and Zhou, Zhengyuan and Leung, Thomas and Li, Li-Jia and Fei-Fei, Li},
  booktitle={Proceedings of the 35th International Conference on Machine Learning},
  pages={2304-2313},
  year={2018},
  publisher = {PMLR},
}
@inproceedings{arpit2017closer,
  title={A closer look at memorization in deep networks},
  author={Arpit, Devansh and Jastrz{\k{e}}bski, Stanis{\l}aw and Ballas, Nicolas and Krueger, David and Bengio, Emmanuel and Kanwal, Maxinder S and Maharaj, Tegan and Fischer, Asja and Courville, Aaron and Bengio, Yoshua and others},
  booktitle={Proceedings of the 34th International Conference on Machine Learning},
  pages={233--242},
  year={2017},
  publisher = {PMLR},
}

@article{zhang2016understanding,
  title={Understanding deep learning requires rethinking generalization},
  author={Zhang, Chiyuan and Bengio, Samy and Hardt, Moritz and Recht, Benjamin and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1611.03530},
  year={2016}
}
@inproceedings{Gulla2017the,
    author = {Gulla, Jon Atle and Zhang, Lemei and Liu, Peng and \"{O}zg\"{o}bek, \"{O}zlem and Su, Xiaomeng},
    title = {The Adressa Dataset for News Recommendation},
    year = {2017},
    publisher = {ACM},
    booktitle = {Proceedings of the International Conference on Web Intelligence},
    pages = {1042–1048}
}

@inproceedings{Yin2013silence,
    author = {Yin, Peifeng and Luo, Ping and Lee, Wang-Chien and Wang, Min},
    title = {Silence is Also Evidence: Interpreting Dwell Time for Recommendation from Psychological Perspective},
    year = {2013},
    publisher = {ACM},
    booktitle = {Proceedings of the 19th SIGKDD International Conference on Knowledge Discovery and Data Mining},
    pages = {989–997},
}
@inproceedings{liu2010understanding,
  title={Understanding web browsing behaviors through Weibull analysis of dwell time},
  author={Liu, Chao and White, Ryen W and Dumais, Susan},
  booktitle={Proceedings of the 33rd international SIGIR Conference on Research and development in information retrieval},
  pages={379--386},
  year={2010},
  organization={ACM}
}
@inproceedings{he2016ups,
    author = {He, Ruining and McAuley, Julian},
    title = {Ups and Downs: Modeling the Visual Evolution of Fashion Trends with One-Class Collaborative Filtering},
    year = {2016},
    publisher = {IW3C2},
    booktitle = {Proceedings of the 25th International Conference on World Wide Web},
    pages = {507–517}
}
@article{duchi2011adaptive,
  title={Adaptive subgradient methods for online learning and stochastic optimization},
  author={Duchi, John and Hazan, Elad and Singer, Yoram},
  journal={Journal of Machine Learning Research},
  volume={12},
  number={Jul},
  pages={2121--2159},
  year={2011}
}
@article{Krizhevsky2017imagenet,
    author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E.},
    title = {ImageNet Classification with Deep Convolutional Neural Networks},
    year = {2017},
    volume = {60},
    number = {6},
    journal = {Communications of the ACM},
    pages = {84–90},
}
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@book{Goodfellow2016deep,
    title={Deep Learning},
    author={Ian Goodfellow and Yoshua Bengio and Aaron Courville},
    publisher={MIT Press},
    year={2016}
}
@inproceedings{Lin2019cross,
    author = {Lin, Tzu-Heng and Gao, Chen and Li, Yong},
    title = {CROSS: Cross-Platform Recommendation for Social E-Commerce},
    year = {2019},
    publisher = {ACM},
    booktitle = {Proceedings of the 42nd International SIGIR Conference on Research and Development in Information Retrieval},
    pages = {515–524},
}


@inproceedings{Yang2018robust,
    author = {Yang, Peng and Zhao, Peilin and Zheng, Vincent W. and Ding, Lizhong and Gao, Xin},
    title = {Robust Asymmetric Recommendation via Min-Max Optimization},
    year = {2018},
    publisher = {ACM},
    booktitle = {The 41st International SIGIR Conference on Research \& Development in Information Retrieval},
    pages = {1077–1080},
}

@inproceedings{Chen2019An,
    author = {Chen, Chong and Zhang, Min and Wang, Chenyang and Ma, Weizhi and Li, Minming and Liu, Yiqun and Ma, Shaoping},
    title = {An Efficient Adaptive Transfer Neural Network for Social-Aware Recommendation},
    year = {2019},
    publisher = {ACM},
    booktitle = {Proceedings of the 42nd International SIGIR Conference on Research and Development in Information Retrieval},
    pages = {225–234}
}
@INPROCEEDINGS{Hu2008CF,
    author={Y. {Hu} and Y. {Koren} and C. {Volinsky}},
    booktitle={Proceedings of the 8th International Conference on Data Mining},
    title={Collaborative Filtering for Implicit Feedback Datasets},
    year={2008},
    pages={263-272},
    publisher={TEEE}
}
@inproceedings{lin2017focal,
    title={Focal loss for dense object detection},
    author={Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
    booktitle={Proceedings of the International Conference on Computer Vision},
    pages={2980--2988},
    year={2017},
    publisher={IEEE}
}
@article{koren2009matrix,
  title={Matrix factorization techniques for Recommender Systems},
  author={Koren, Yehuda and Bell, Robert and Volinsky, Chris},
  journal={Computer},
  number={8},
  volume={42},
  pages={30--37},
  year={2009},
  publisher={IEEE}
}
@inproceedings{mnih2008probabilistic,
  title={Probabilistic matrix factorization},
  author={Mnih, Andriy and Salakhutdinov, Ruslan R},
  booktitle = {Proceedings of the 22nd International Conference on Neural Information Processing Systems},
  pages={1257--1264},
  year={2008},
  publisher = {MIT Press}
}

@inproceedings{Koren2008Factorization,
    author = {Koren, Yehuda},
    title = {Factorization Meets the Neighborhood: A Multifaceted Collaborative Filtering Model},
    year = {2008},
    publisher = {ACM},
    booktitle = {Proceedings of the 14th SIGKDD International Conference on Knowledge Discovery and Data Mining},
    pages = {426–434}
}

@article{Rosasco2004are,
    author = {Rosasco, Lorenzo and De Vito, Ernesto and Caponnetto, Andrea and Piana, Michele and Verri, Alessandro},
    title = {Are Loss Functions All the Same?},
    year = {2004},
    publisher = {MIT Press},
    volume = {16},
    number = {5},
    journal = {Neural Computation.},
    pages = {1063–1076}
}
@inproceedings{rendle2009bpr,
  title={BPR: Bayesian personalized ranking from implicit feedback},
  author={Rendle, Steffen and Freudenthaler, Christoph and Gantner, Zeno and Schmidt-Thieme, Lars},
  booktitle={Proceedings of the 25th Conference on Uncertainty in Artificial Intelligence},
  pages={452--461},
  year={2009},
  publisher={AUAI Press}
}

@inproceedings{gao2019neural,
  title={Neural multi-task recommendation from multi-behavior data},
  author={Gao, Chen and He, Xiangnan and Gan, Dahua and Chen, Xiangning and Feng, Fuli and Li, Yong and Chua, Tat-Seng and Jin, Depeng},
  booktitle={Proceedings of the 35th International Conference on Data Engineering},
  pages={1554--1557},
  year={2019},
  publisher={IEEE}
}

@article{Gao2019LearningTR,
  title={Learning to Recommend with Multiple Cascading Behaviors},
  author={Chen Gao and Xiangnan He and Dahua Gan and Xiangning Chen and Fuli Feng and Yueming Li and Tat-Seng Chua and Lina Yao and Yang Song and Depeng Jin},
  journal={Transactions on Knowledge and Data Engineering},
  year={2019},
  publisher={IEEE}
}

@article{ding2019sampler,
  title={Sampler design for bayesian personalized ranking by leveraging view data},
  author={Ding, Jingtao and Yu, Guanghui and He, Xiangnan and Feng, Fuli and Li, Yong and Jin, Depeng},
  journal={Transactions on Knowledge and Data Engineering},
  year={2019},
  publisher={IEEE}
}

@inproceedings{Hofmann2012on,
    author = {Hofmann, Katja and Behr, Fritz and Radlinski, Filip},
    title = {On Caption Bias in Interleaving Experiments},
    publisher = {ACM},
    year = {2012},
    booktitle = {Proceedings of the 21st International Conference on Information and Knowledge Management},
    pages = {115–124}
}

@inproceedings{Bengio2009Curriculum,
    author = {Bengio, Yoshua and Louradour, J\'{e}r\^{o}me and Collobert, Ronan and Weston, Jason},
    title = {Curriculum Learning},
    year = {2009},
    booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
    pages = {41–48},
    publisher = {ACM}
}


@inproceedings{lambdaopt,
 author = {Chen, Yihong and Chen, Bei and He, Xiangnan and Gao, Chen and Li, Yong and Lou, Jian-Guang and Wang, Yue},
 title = {lambdaOpt: Learn to Regularize Recommender Models in Finer Levels},
 booktitle = {Proceedings of the 25th SIGKDD International Conference on Knowledge Discovery and Data Mining},
 year = {2019},
 pages = {978--986},
 publisher = {ACM},
} 

@inproceedings{LightGCN2020he,
    author = {He, Xiangnan and Deng, Kuan and Wang, Xiang and Li, Yan and Zhang, YongDong and Wang, Meng},
    title = {LightGCN: Simplifying and Powering Graph Convolution Network for Recommendation},
    year = {2020},
    publisher = {ACM},
    booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
    pages = {639–648}
}
@article{chen2020bias,
  title={Bias and Debias in Recommender System: A Survey and Future Directions},
  author={Jiawei Chen and Hande Dong and Xiang Wang and Fuli Feng and Meng Wang and Xiangnan He},
  year={2020},
  journal={arXiv preprint arXiv:2010.03240}
}


@article{wang2020click,
  title={"Click" Is Not Equal to "Like": Counterfactual Recommendation for Mitigating Clickbait Issue},
  author={Wang, Wenjie and Feng, Fuli and He, Xiangnan and Zhang, Hanwang and Chua, Tat-Seng},
  journal={arXiv preprint arXiv:2009.09945},
  year={2020}
}

@inproceedings{jiang2020aspect,
  title={What Aspect Do You Like: Multi-scale Time-aware User Interest Modeling for Micro-video Recommendation},
  author={Jiang, Hao and Wang, Wenjie and Wei, Yinwei and Gao, Zan and Wang, Yinglong and Nie, Liqiang},
  booktitle={Proceedings of the 28th ACM International Conference on Multimedia},
  pages={3487--3495},
  year={2020},
  publisher={ACM}
}

@inproceedings{wang2018chat,
  title={Chat more: Deepening and widening the chatting topic via a deep model},
  author={Wang, Wenjie and Huang, Minlie and Xu, Xin-Shun and Shen, Fumin and Nie, Liqiang},
  booktitle={The 41st International ACM SIGIR Conference on Research \& Development in Information Retrieval},
  pages={255--264},
  year={2018},
  publisher={ACM}
}

@inproceedings{nie2019multimodal,
  title={Multimodal dialog system: Generating responses via adaptive decoders},
  author={Nie, Liqiang and Wang, Wenjie and Hong, Richang and Wang, Meng and Tian, Qi},
  booktitle={Proceedings of the 27th ACM International Conference on Multimedia},
  pages={1098--1106},
  year={2019},
  publisher={ACM}
}

@article{Cheng2019MMALFM,
    author = {Cheng, Zhiyong and Chang, Xiaojun and Zhu, Lei and Kanjirathinkal, Rose C. and Kankanhalli, Mohan},
    title = {MMALFM: Explainable Recommendation by Leveraging Reviews and Images},
    year = {2019},
    publisher = {ACM},
    volume = {37},
    number = {2},
    journal = {ACM Trans. Inf. Syst.},
    month = jan,
    articleno = {16}
}

@inproceedings{ren2017social,
  title={Social collaborative viewpoint regression with explainable recommendations},
  author={Ren, Zhaochun and Liang, Shangsong and Li, Piji and Wang, Shuaiqiang and de Rijke, Maarten},
  booktitle={Proceedings of the tenth ACM international conference on web search and data mining},
  pages={485--494},
  year={2017},
  publisher = {ACM}
}
